On The Decoding Error Weight of One or Two Deletion Channels

This paper tackles two problems that fall under the study of coding for insertions and deletions. These problems are motivated by several applications, among them is reconstructing strands in DNA-based storage systems. Under this paradigm, a word is transmitted over some fixed number of identical independent channels and the goal of the decoder is to output the transmitted word or some close approximation of it. The first part of the paper studies optimal decoding for a special case of the deletion channel, referred by the $k$-deletion channel, which deletes exactly $k$ symbols of the transmitted word uniformly at random. In this part, the goal is to understand how an optimal decoder operates in order to minimize the expected normalized distance. A full characterization of an efficient optimal decoder for this setup, referred to as the maximum likelihood* (ML*) decoder, is given for a channel that deletes one or two symbols. The second part of this paper studies the deletion channel that deletes a symbol with some fixed probability $p$, while focusing on two instances of this channel. Since operating the maximum likelihood (ML) decoder, in this case, is computationally unfeasible, we study a slightly degraded version of this decoder for two channels and study its expected normalized distance. We observe that the dominant error patterns are deletions in the same run or errors resulting from alternating sequences. Based on these observations, we derive lower bounds on the expected normalized distance of the degraded ML decoder for any transmitted $q$-ary sequence of length $n$ and any deletion probability $p$. We further show that as the word length approaches infinity and the channel's deletion probability $p$ approaches zero, these bounds converge to approximately $\frac{3q - 1}{q - 1} p^2$. These theoretical results are verified by corresponding simulations.

==> 5-2del2ins.tex <==
\section{Two Deletion Channels}\label{sec:two deletions}

In this section we study the case of two instances of the deletion channel, $\del(p)$, where every symbol is deleted with probability $p$. % and prove in Theorem~\ref{th:2ch} an approximation for the expected normalized distance in the form of $$\perr(q,p) \approx \frac{3q-1}{q-1}p^2 + O(p^3).$$
%Complexity wise, it is well known that the time complexity to calculate the SCS length and the embedding numbers of two sequences are both quadratic with their length. However, the number of SCSs can grow exponentially~\cite{itoga1981string, elzinga2008algorithms}.  Thus, given a list of SCSs of size $L$, the complexity of the ML decoder for $t=2$ will be $O(Ln^2)$. The main idea behind these algorithms uses dynamic programming in order to calculate the SCS length and the embedding numbers for all prefixes of the given words. However, when calculating for example the SCS for $\bfy_1$ and $\bfy_2$ it is already known that $\mathsf{SCS}(\bfy_1,\bfy_2) \leq n$. Hence, it is not hard to observe that (see e.g.~\cite{apostolico1992fast}) many paths corresponding to prefixes which their length difference is greater than $d_1+d_2$ can be eliminated, when $d_1,d_2$ is the number of deletions in $\bfy_1,\bfy_2$, respectively. In particular, when $d_1$ and $d_2$ are fixed, then the time complexity is linear. In our simulations we used this improvement when implementing the ML decoder. Other improvements and algorithms of the ML decoder are discussed in~\cite{srinivasavaradhan2018maximum,srinivasavaradhan2019symbolwise}.
Recall that for a given codeword $\bfc \in \cC$ and two channel outputs  $\bfy_1, \bfy_2 \in (\Sigma_q)^{\leq |\bfc|}$, by Claim~\ref{cl:ML*multiple}, the output of the ML$^*$ decoder is
\begin{align*}
\cD_{\ML^*}(\bfy_1, \bfy_2) = \argmin_{\bfx\in \Sigma_q^*} \left\{\sum_{\substack{\bfc \in \cC \\ \bfc \in \sups (\bfy_1, \bfy_2 )}}  {d_L(\bfx,\bfc) \prod_{i=1}^2 \emb(\bfc ; \bfy_i)}\right\}. 
\end{align*}
Since the number of shorterst common supersequences of $\bfy_1$ and $\bfy_2$ can grow exponentially with their lengths~\cite{itoga1981string}, a direct computation of the ML$^*$ decoder might be impractical in this case. Hence, not only that the number of candidates $\bfx$ is infinite, the number of codewords  $\bfc\in \cC \cap \sups (\bfy_1, \bfy_2 )$ that are evaluated in the summation can be exponential. Therefore, we suggest a suboptimal approach, which is yet very practical. Instead of using the formal definition of the ML$^*$ decoder, in this section a degraded version of the ML$^*$ decoder is used. \textcolor{blue}{The decoder is designed with a limitation that may result in producing an output that is not necessarily a codeword, but rather a word of shorter length.} This decoder, denoted by $\cD_{\ML^D}$ and referred as the ML$^D$ \emph{decoder}, is defined as follows
%the following definition, that approximates the ML$^*$ decoder. For convenience, we keep it under the same notation of the ML$^*$ decoder. 
\begin{align*}
 \cD_{\ML^D}(\bfy_1, \bfy_2) = \argmax_{\bfx\in \sups(\bfy_1, \bfy_2)} \left\{ \emb(\bfx ; \bfy_1) \emb(\bfx ; \bfy_2)\right\}. 
\end{align*}

Assume $\cC$ is $\Sigma_q^n$. The average decoding failure probability of the ML$^D$ decoder over two deletion channels $\del(p)$ is denoted by $\pfail(q,p)$. Similarly, the expected normalized distance is denoted by $\perr(q,p)$. These values provide upper bounds on the corresponding error probabilities of the ML$^*$ decoder. Our main goal in this section is to calculate close approximations for $\pfail(q,p)$ and $\perr(q,p)$. Note that a lower bound on these probabilities is $p^2$ (and more generally $p^t$ for $t$ channels) since if the same symbol is deleted in all of the channels, then it is not possible to recover its value and thus it will be deleted also in the output of the ML$^D$ decoder. This was already observed in~\cite{srinivasavaradhan2018maximum} and in their simulation results. We will also analyze these failure and error probabilities for the VT code\cite{VT} and the SVT code~\cite{7837631}.

The lower bound $p^2$ on $\perr(q,p)$ is not tight since if symbols from the same run are deleted then the outputs of the two channels of this run are the same and it is impossible to detect that this run experienced a deletion in both of its copies. The error probability due to deletions within runs is denoted by $\prun(q,p)$ and the next lemma approximates this probability. 
%We let $\alpha_{t,q}$ be the value $$\alpha_{t,q}=\sum_{r=1}^{\infty} r^t \left(\frac{1}{q}\right)^{r-1},$$  so $\alpha_{2,q} = \frac{q^2(q+1)}{(q-1)^3}$, $\alpha_{3,q} = \frac{q^4+4q^3+q^2}{(q-1)^4}$, and $\alpha_{4,q} = \frac{q^5+11q^4+11q^3+q^2}{(q-1)^5}$.
\begin{lemma} \label{lm:2ch_run_del}
For the deletion channel $\del(p)$, it holds that 
%It holds that The average deletion probability of the ML decoder's output because of the runs is at least 
$$\prun(q,p)  \approx \frac{q+1}{q-1}p^2.$$
\end{lemma}
\begin{IEEEproof} 
Given a run of length $r$, the probability that both of its copies have experienced a deletion is roughly $(rp)^2$. Furthermore, the occurrence probability of a run of length exactly $r$ is $ \frac{q-1}{q} \cdot \left(\frac{1}{q}\right)^{r-1}$. Thus, for $n$ large enough, the error probability is approximated by 
\begin{align*}
\sum_{r=1}^{\infty} (rp)^2 \cdot  \frac{q-1}{q} \cdot \left(\frac{1}{q}\right)^{r-1} &= p^2\cdot \frac{q-1}{q} \sum_{r=1}^{\infty} r^2 \left(\frac{1}{q}\right)^{r-1} & \\
& = p^2\cdot \frac{q-1}{q} \frac{1+\frac{1}{q}}{(1-\frac{1}{q})^3} = p^2\cdot \frac{q(q+1)}{(q-1)^2}.& 
\end{align*}
The expected length of a run is given by 
$$\sum_{r=1}^{\infty} r \left(\frac{1}{q}\right)^{r-1}\cdot\frac{q-1}{q} =\frac{q-1}{q} \sum_{r=1}^{\infty} r \left(\frac{1}{q}\right)^{r-1} = \frac{q}{q-1}.$$
Hence, the expected number of runs in a vector of length $n$ is $n\cdot \frac{q-1}{q}$ and thus the approximated number of deletions in the decoder's output due to runs is 
$$n\cdot \frac{q-1}{q} \cdot p^2\cdot \frac{q(q+1)}{(q-1)^2} = n p^2\cdot  \frac{q+1}{q-1},$$
which verifies the statement in the lemma. \end{IEEEproof}
%Another proof works as follows. Assume that the close deletions in the two copies are in positions $i$ and $i+j$. Then, there is a run deletion if there is a run between positions $i$ and $i+j$, which happens with probability $p1/q^j$. Hence, the deletion probability because of the runs is $$p^2\left(1 + 2\sum_{j=1}^\infty \frac{1}{q^j}\right)  = p^2\left(1 + \frac{2}{q-1}\right) = \frac{q+1}{q-1}p^2.$$


However, runs are not the only source of errors in the output of the ML$^D$ decoder. For example, assume the $i$-th and the $(i+1)$-st symbols are deleted from the first and the second channel output, respectively. If the transmitted word $\bfx$ is of the form $\bfx = (x_1,\ldots,x_{i-1},0,1,x_{i+2},\ldots,x_n)$, then the two channels' outputs are $\bfy_1 = (x_1,\ldots,x_{i-1},0,x_{i+2},\ldots,x_n)$ and $\bfy_2 = (x_1,\ldots,x_{i-1},1,x_{i+2},\ldots,x_n)$. However, these two outputs could also be received upon deletions exactly in the same positions if the transmitted word was $\bfx' = (x_1,\ldots,x_{i-1},1,0,x_{i+2},\ldots,x_n)$. Hence, the ML$^D$ decoder can output the correct word only in one of these two cases. Longer alternating sequences cause the same problem as well and the \emph{occurrence} probability of this event, denoted by $\palt(q,p)$, will be estimated in the next lemma. 
%This scenario extended to any alternating sequence, as will be shown in the next lemma. The error probability of this event is denoted by $\palt(q,p)$
\begin{lemma} \label{lm:2ch_alt_del}
For the deletion channel $\del(p)$, it holds that 
%It holds that The average deletion probability of the ML decoder's output because of the runs is at least 
$$\palt(q,p)  \approx 2p^2.$$
\end{lemma} 
\begin{IEEEproof}
\begin{comment}
Assume that 


Given a run of length $r$, the probability that both of its copies have experience a deletion is at lease $(rp)^2$. Furthermore, the occurrence probability of a run of length exactly $r$ is $\left(\frac{1}{q}\right)^{r-1}\cdot\frac{q-1}{q}$. Thus, for $n$ large enough, the error probability is approximated by 
\begin{align*}
\sum_{r=1}^{\infty} (rp)^2  \left(\frac{1}{q}\right)^{r-1}&\cdot\frac{q-1}{q} = p^2\cdot \frac{q-1}{q} \sum_{r=1}^{\infty} r^2 \left(\frac{1}{q}\right)^{r-1} & \\
& = p^2\cdot \frac{q-1}{q} \frac{1+\frac{1}{q}}{(1-\frac{1}{q})^3} = p^2\cdot \frac{q(q+1)}{(q-1)^2}.& 
\end{align*}
The expected length of a run is given by 
$$\sum_{r=1}^{\infty} r \left(\frac{1}{q}\right)^{r-1}\cdot\frac{q-1}{q} =\frac{q-1}{q} \sum_{r=1}^{\infty} r \left(\frac{1}{q}\right)^{r-1} = \frac{q}{q-1}.$$
Hence, the expected number of runs in a vector of length $n$ is $n\cdot \frac{q-1}{q}$ and thus the approximated number of deletions due to runs is 
$$n\cdot \frac{q-1}{q} \cdot p^2\cdot \frac{q(q+1)}{(q-1)^2} = n p^2\cdot  \frac{q+1}{q-1},$$
which verifies the statement in the lemma. 
\end{comment}
Assume there is a deletion in the first channel in the $i$-th position and the closest deletion in the second channel is $j>0$ positions apart, i.e., either in position $i-j$ or $i+j$. W.l.o.g. assume it is in the $(i+j)$-th position and $\bfx_{[i:j]}$ is an alternating sequence $ABAB\cdots$. Then, the 
%Assume that the close deletions in the two copies are in positions $i$ and $i+j$ and $\bfx_{[i:j]}$ is an alternating sequence. 
same outputs from the two channels could be received if the transmitted word was the same as $\bfx$ but with the opposite order of the symbols of the alternating sequence, that is, the symbols of the word in the positions of $[i:j]$ are $BABA\cdots$. Therefore, the occurrence probability of this event can be approximated by
$$2p^2\cdot \sum_{j=1}^\infty \frac{q-1}{q}\cdot \frac{1}{q^{j-1}} = 2p^2,$$
where  $\frac{q-1}{q}\cdot \frac{1}{q^{j-1}}$ is the probability that $\bfx_{[i:j]}$ is any alternating sequence and the multiplication by 2 takes into account the cases of deletion in either position $i-j$ or $i+j$.
\end{IEEEproof}

%At this point one may ask whether these two error events are the only dominant ones and indeed this question is answered in the affirmative, as stated in the following lemma. 


\begin{comment}
\begin{lemma}
If there are deletions in positions $i$ and $i+c$ for $c\geq 1$, and $\bfx_{[i:i+c]}$ is an alternating sequence. Then the  the same traces are obtained for $x$  and for ${x'}=(\bfx_{[0:i-1},\ceil{\bfx_{[i:i+c]}}, \bfx_{[i+c+1,n]})$, where $\ceil{\bfx_{[i:i+c]}}$ represent the complement of the alternating sequence $\bfx_{[i:i+c]}$. 
\end{lemma}
\begin{IEEEproof}
\e{Assume that $c$ is odd and furthermore $\bfx_{[i:i+c]}  =(A,B,A,B,\ldots,A,B)$ so the two channel outputs on this interval of $\bfx$ are $(B,A,B,\ldots,A,B)$ and $(A,B,A,B,\ldots,A)$. These two outputs could also be received if $\bfx_{[i:i+c]}  =(B,A,B,\ldots,A,B,A)$ and thus the ML decoder cannot distinguish between these two cases. The same proof hold in case $c$ is even.}
\end{IEEEproof}
\begin{corollary}
Given a transmitted word of the shape of $x=(\bfx_{[0:i-1},\bfx_{[i:i+c]}, \bfx_{[i+c+1,n]})$, where $\bfx_{[i:i+c]}$ is an alternating sequence. And given that there are deletions in positions $i$ and $i+c$, the ${ML}^*$ decoder fails in probability of 0.5. This failure is resulted in 2 Levenshtein errors.  
\end{corollary}
\begin{IEEEproof}
\e{TO BE Completed...}
\end{IEEEproof}
\end{comment}
\begin{comment}
\begin{lemma} 
Assume there is a deletion in the first, second channel in position $i, i+j$, where $j>0$, where $i$, $i+j$ is the right most position, left most position, within its run, respectively. If the sequence $\bfx_{[i:i+j]}$ is neither a run nor an alternating sequence, then these deletions are corrected successfully by the ML$^D$ decoder. 
%If there are deletions in positions $i$ and $i+c$ for $c\geq 1$, and the transmitted word is of the shape of $x=(\bfx_{[0:i-1},\bfx_{[i:i+c]}, \bfx_{[i+c+1,n]}$, where $\bfx_{[i:i+c]}$ is not the alternating sequence or a run, then the ${ML}^*$ decoder can successfully decode the word $x$. 
\end{lemma}
%\begin{comment}
\begin{IEEEproof}
\e{The output of the first channel from the bits in positions between $i$ and $i+j$ is $(x_{i+1},x_{i+2},\ldots,x_{i+j})$ and the output of the second channel in these positions is $(x_{i},x_{i+1},\ldots,x_{i+j-1})$. Clearly, it holds that $(x_i,x_{i+1},x_{i+2},\ldots,x_{i+j})$ is a candidate for the ML$^D$ decoder. If another vector $(x_i',x_{i+1}',x_{i+2}',\ldots,x_{i+j}')$ is also a candidate for the ML$^D$ decoder, it should hold that $$(x_i',x_{i+1}',x_{i+2}',\ldots,x_{i+j-1}') = (x_{i+1},x_{i+2},\ldots,x_{i+j})$$
and  
$$(x_{i+1}',x_{i+2}',\ldots,x_{i+j}') = (x_{i},x_{i+1},\ldots,x_{i+j-1}).$$
Therefore we get that $x_i'=x_{i+2}'=x_{i+4}'=\cdots $ and $x_{i+1}'=x_{i+3}'=x_{i+5}'=\cdots $, i.e., $\bfx_{[i:i+j]}$ is either the alternating sequence or a run, which results with a contradiction.}

\e{Let us assume in contradiction that $\bfx_{[i:i+j]}$ is not the alternating sequence and not a single run, but still there is more than one candidate to the ML$^D$ decoder. The output of the first channel ${\bfy_1}_{[i:i+j-1]}$ (between indices $i$ and $i+j-1$) is $(x_{i+1},x_{i+2},\ldots,x_{i+j})$. Similarly, the output of the second channel ${\bfy_2}_{[i:i+j-1]}$ in these indices is $(x_{i},x_{i+1},\ldots,x_{i+j-1})$.  By Lemma~\ref{},  and since  $\bfx_{[i:i+j]}$ is not a run, and therefore ${\bfy_1}_{[i:i+j-1]} \ne {\bfy_2}_{[i:i+j-1]}$, it holds that the shortest common supersequence of ${\bfy_1}_{[i:i+j-1]}$ and ${\bfy_2}_{[i:i+j-1]}$ is a sequence from the set $I_1({\bfy_1}_{[i:i+j-1]}) \cap I_1({\bfy_2}_{[i:i+j-1]}$), that is, the sequence is obtained from ${\bfy_1}_{[i:i+j-1]}$, and from ${\bfy_2}_{[i:i+j-1]}$ by inserting one symbol. Clearly, $\bfx_{[i:i+j]} \in I_1({\bfy_1}_{[i:i+j-1]}) \cap I_1({\bfy_2}_{[i:i+j-1]}$, let us assume that there is another sequence $\bfx' \in  I_1({\bfy_1}_{[i:i+j-1]}) \cap I_1({\bfy_2}_{[i:i+j-1]}$, such that $p(\bfy_1, \bfy_2 | \bfx')= p(\bfy_1, \bfy_2 | \bfx')$. Let us assume that $\bfx'$ is obtained from ${\bfy_1}_{[i:i+j-1]}$ by inserting the symbol $\alpha$ after the index $i+h$, or by inserting the symbol $\beta$ after the index $i+h'$ to the word ${\bfy_2}_{[i:i+j-1]}$}

\e{First we note that the errror probability of any error event of the ML$^D$ decoder that is resulted from 3 or more errors in the two channel outputs between the $i$ and the $i+j$ indices error probability is proportion to $p^3$. Hence, we can deduce that there were $2$ deletions in the two copies and that we have one deletion in each channel output (otherwise there is a noiseless channel output that can be the decoder's output). Let $\bfy_1$ and $\bfy_2$ be the channel outputs, from the Lemma's assumption, it is known that the deletion of the $i$-th symbol of $\bfy_1$ and the deletion of the $i+j$-th symbol of  $\bfy_2$ are deletions from two different runs of the transmitted word.  }
\end{IEEEproof}
\end{comment}
%\end{comment}
%\end{comment}
\begin{comment}
However, runs are not the only source of errors in the ML decoder. For example, assume the $i$-th, $(i+1)$-th bit is deleted in the first, second channel, respectively. If $(x_i,x_{i+1}) = (0,1)$, then a decoder cannot distinguish whether the values of these two bits in the transmitted work are $(0,1)$ or $(1,0)$. This is extended to any alternating sequence, as will be shown in the next lemma. 
\begin{lemma}
If there are deletions in positions $i$ and $i+c$ for $c\geq 1$, and $\bfx_{[i:i+c]}$ is an alternating sequence, then the ML decoder cannot distinguish between $\bfx_{[i:i+c]}$ and its complement. 
\end{lemma}
\begin{IEEEproof}
Assume that $c$ is odd and furthermore $\bfx_{[i:i+c]}  =(A,B,A,B,\ldots,A,B)$ so the two channel outputs on this interval of $\bfx$ are $(B,A,B,\ldots,A,B)$ and $(A,B,A,B,\ldots,A)$. These two outputs could also be received if $\bfx_{[i:i+c]}  =(B,A,B,\ldots,A,B,A)$ and thus the ML decoder cannot distinguish between these two cases. The same proof hold in case $c$ is even.
\end{IEEEproof}

\begin{lemma}
If there are deletions in positions $i$ and $i+c$ for $c\geq 1$, and $\bfx_{[i:i+c]}$ is not the alternating sequence or a run, then the ML decoder can successfully decode $\bfx_{[i:i+c]}$. 
\end{lemma}
\begin{IEEEproof}
The output of the first channel is $(x_{i+1},x_{i+2},\ldots,x_{i+c})$ and the one of the second channel is $(x_{i},x_{i+1},\ldots,x_{i+c-1})$. Clearly, it holds that $(x_i,x_{i+1},x_{i+2},\ldots,x_{i+c})$ is a candidate for the ML decoder. If  the vector $(x_i',x_{i+1}',x_{i+2}',\ldots,x_{i+c}')$ is another candidate for the ML decoder, it should hold that $$(x_i',x_{i+1}',x_{i+2}',\ldots,x_{i+c-1}') = (x_{i+1},x_{i+2},\ldots,x_{i+c})$$
and  
$$(x_{i+1}',x_{i+2}',\ldots,x_{i+c}') = (x_{i},x_{i+1},\ldots,x_{i+c-1}).$$
Therefore we get that $x_i'=x_{i+2}'=x_{i+4}'=\cdots $ and $x_{i+1}'=x_{i+3}'=x_{i+5}'=\cdots $, i.e., $\bfx_{[i:i+c]}$ is either the alternating sequence or a run, which results with a contradiction. 
\end{IEEEproof}
\end{comment}


\begin{comment}

The following notations will be used in the next lemma. We denote by $n'$ the number of alternating segments in $\bfx$ and by $n''$  the number of runs of length at least two in $\bfx$. Additionally, we denote by $i_1, i_2, \ldots i_{n'}$ the indices of the first symbol of each of the alternating segments in $\bfx$ and by $j_1, j_2, \ldots, j_{n''}$ the indices of the first symbol of each run of length at least two in $\bfx$.


\begin{lemma} 
If the channel outputs $\bfy_1$ and $\bfy_2$ can be obtained from $\bfx$ such that in each alternating segement and in each run of length at least two there is a deletion in at most one channel output ($\bfy_1$ or $\bfy_2$, but not in both of them). Then $\bfy_1$ and $\bfy_2$ has  exactly one SCS, which is $\bfx$ and therefore in that case the $ML^D$ outputs the correct word. 
 \end{lemma}
 
 \begin{IEEEproof}
 First, note that if the two channel outputs are obtained from $\bfx$ by deleting symbols from two consecutive runs, or from two non-consecutive runs such that the sequence between these two run is an alternating segment, this is equivalent to the case where there are deletions from the alternating sequence in each one of them. Hence, we can consider only cases where there are deletions from two non-consecutive runs, such that there is at least one run of length at least two between them. 
Assume to the contrary that $\bfy_1$ and $\bfy_2$ can be obtained from $\bfx$ by deleting symbols from $\bfx$ such that the lemma's condition holds, but there is more the one SCSs for $\bfy_1$ and $\bfy_2$.  Let $\bfx_1$ and $\bfx_2$ be two different SCSs of $\bfy_1$ and $\bfy_2$, from the definition we get that $|\bfx_1|=|\bfx_2|$ and that both of them are supersequences of $\bfy_1$ and $\bfy_2$. Recall that $\rho(\bfx)$ dentoes the number of run in $\bfx$, since $\bfx_1 \ne \bfx_2$, we have one of the following distinct cases: 
\begin{enumerate}
\item \textbf{Case 1:} $\rho(\bfx_1) \ne \rho(\bfx_2)$, in this case we assume w.l.o.g. that $\rho(\bfx_1) > \rho(\bfx_2)$, that is there is at lease one run in $\bfx_1$ that does not appear in $\bfx_2$. Since we assume that 
\item \textbf{Case 1:} $\rho(\bfx_1) = \rho(\bfx_2)$, in this case there is at least one run that is longer in $\bfx_1$ compare to $\bfx_2$. Assume that this run  Since we assume that 

\end{enumerate}

\end{comment}
\begin{comment}
The following notations will be used in the next lemma. For the transmitted word $\bfx$, we denote by $\rho(\bfx)$ the number of runs in $\bfx$. For the channel outputs $\bfy_1$ and $\bfy_2$, we denote by $\rho_1$ and $\rho_2$ the number of runs that were shortened in $\bfx$ in order to obtain $\bfy_1$ and $\bfy_2$, respectively. We further denote by $i_1 < i_2 < \ldots < i_{\rho_1}$ the sorted set of indices of the runs in $\bfx$ that were shortened or deleted in order to obtain $\bfy_1$, the sorted set of these indices is denotes by $\cI$. Similarly, $j_1 <  j_2 < \ldots < j_{\rho_2}$ denote these runs in $\bfy_2$, and their set is denoted by $\cJ$. Note that $1 < i_h, j_\ell < \rho(\bfx)$ for any $1 \le h \le \rho_1 $ and $1 \le \ell \le \rho_2$. The following lemma states that if for any pair of indices $i_h$ and $j_\ell$, $i_h \ne j_\ell$, there is at least one run from $\bfx$ of length at least two, such that none of its symbols were deleted neither in $\bfy_1$ nor in $\bfy_2$, it holds that the word $\bfx$ can be decoded uniquely.

\begin{lemma} 
If for any pair of indices $i_h$ and $j_\ell$, $i_h \ne j_\ell$, there is at least one run from $\bfx$ of length at least two, such that none of its symbols were deleted neither in $\bfy_1$ nor in $\bfy_2$, it holds that the word $\bfx$ can be decoded uniquely.
 \end{lemma}
 
 \begin{IEEEproof}
In the following proof we will show a constructive determinstic decoder that can decode the transmitted word $\bfx$.
Given the two disjoint sets $\cI$ and $\cJ$, we recall that from the lemma assumption, for any two indices $i_h\in \cI$ and $j_{\ell} \in \cJ$, it holds that there is at lease one run of length at least two, such that none of its symbols were deleted neither in $\bfy_1$ nor in $\bfy_2$. The following steps describe how the decoder can reconstruct the word $\bfx$. In each iteration, the decoder selects the smallest indices $i_h$ and $j_{\ell}$, such that w.l.o.g. $i_h < j_{\ell}$ and for any $i_{h'} > i_{h}$, it holds that $i_{h'} > j_{\ell}$. From the induction assumption it holds that any symbol prior the $i_{h}$ run was reconstructed correctly by the decoder, therefore the decoder can  that are  lemma's assumption it holds that 


\begin{enumerate}
\item \textbf{Case 1:} $\rho(\bfx_1) \ne \rho(\bfx_2)$, in this case we assume w.l.o.g. that $\rho(\bfx_1) > \rho(\bfx_2)$, that is there is at lease one run in $\bfx_1$ that does not appear in $\bfx_2$. Since we assume that 
\item \textbf{Case 1:} $\rho(\bfx_1) = \rho(\bfx_2)$, in this case there is at least one run that is longer in $\bfx_1$ compare to $\bfx_2$. Assume that this run  Since we assume that 
\end{enumerate}
%First, note that if the two channel outputs are obtained from $\bfx$ by deleting symbols from two consecutive runs, or from two non-consecutive runs such that the sequence between these two run is an alternating segment, this is equivalent to the case where there are deletions from the alternating sequence in each one of them. Hence, we can consider only cases where there are deletions from two non-consecutive runs, such that there is at least one run of length at least two between them. 
%Assume to the contrary that $\bfy_1$ and $\bfy_2$ can be obtained from $\bfx$ by deleting symbols from $\bfx$ such that the lemma's condition holds, but there is more the one SCSs for $\bfy_1$ and $\bfy_2$.  Let $\bfx_1$ and $\bfx_2$ be two different SCSs of $\bfy_1$ and $\bfy_2$, from the definition we get that $|\bfx_1|=|\bfx_2|$ and that both of them are supersequences of $\bfy_1$ and $\bfy_2$. Recall that $\rho(\bfx)$ dentoes the number of run in $\bfx$, since $\bfx_1 \ne \bfx_2$, we have one of the following distinct cases: 
%\begin{enumerate}
%\item \textbf{Case 1:} $\rho(\bfx_1) \ne \rho(\bfx_2)$, in this case we assume w.l.o.g. that $\rho(\bfx_1) > \rho(\bfx_2)$, that is there is at lease one run in $\bfx_1$ that does not appear in $\bfx_2$. Since we assume that 
%\item \textbf{Case 1:} $\rho(\bfx_1) = \rho(\bfx_2)$, in this case there is at least one run that is longer in $\bfx_1$ compare to $\bfx_2$. Assume that this run  Since we assume that 
 
 
\end{IEEEproof}
\end{comment}

It should be noted that the approximation of $\prun(q,p)$, $\palt(q,p)$ that was proved in Lemma~\ref{lm:2ch_run_del}, Lemma~\ref{lm:2ch_alt_del} is in fact an upper bound on this value at our simulations, respectively. This can be explained due to the fact that in these approximations we consider runs and alternating sequences of any length. However, when the code is $\cC=\Sigma_q^n$, almost all of the codewords do not have long runs or long alternating sequences (for example of length that is $\theta (n)$), and hence some of these error events are extremely rare and most likely were not generated in our simulations. Moreover, the probability to have long runs and long alternating sequences decreases as $q$ increases. This observation can also be seen in our simulations in Figures~\ref{fig:LER-Deletion} and~\ref{fig:runAltErrorsDel}. On the other hand, these lemmas neglect any error event that involves more than a single deletion in a specific run or a specific alternating sequence in one of the channel outputs. These error events do increase the error probability of the decoder, but their probability is $O(p^3)$. As a conclusion from Lemma~\ref{lm:2ch_run_del} and Lemma~\ref{lm:2ch_alt_del}, we can approximate the expected normalized distance for the case of two deletion channels to be the sum of the Levenshtein error rate due to errors in runs (Lemma~\ref{lm:2ch_run_del}), the Levenshtein error rate due to alternating sequence errors (Lemma~\ref{lm:2ch_alt_del}), and additional errors which are in the order of $p^3$. Hence, the expected normalized distance of the ML$^D$ decoder for the case of two deletion channels is approximated by 
$$\perr(q,p) \lesssim \prun(q,p) + \palt(q,p)+O(p^3) = \frac{3q-1}{q-1}p^2+O(p^3).$$
%The following theorem, which approximates the Levenshtein error rate for the case of two deletion channels is a conclusion from Lemma~\ref{} and Lemma~\ref{}.
%We are now ready to show the following theorem on the Levenshtein error rate for the case of two channels. 
\begin{comment}
\begin{theorem}\label{th:2ch}
The Levenshtein error rate for two deletion channels is approximated by 
$$\hspace{-0.3ex}\perr(q,\hspace{-0.25ex}p)\hspace{-0.35ex} \approx\hspace{-0.35ex} \prun(q,\hspace{-0.25ex}p) \hspace{-0.3ex}+\hspace{-0.3ex} \palt(q,\hspace{-0.25ex}p) \hspace{-0.3ex}+\hspace{-0.3ex}O(p^3) \hspace{-0.3ex}=\hspace{-0.3ex} \frac{3q\hspace{-0.3ex}-\hspace{-0.3ex}1}{q\hspace{-0.3ex}-\hspace{-0.3ex}1}p^2\hspace{-0.3ex}+\hspace{-0.3ex}O(p^3).$$
\end{theorem}
\begin{IEEEproof}
\e{First we note that the error probability of any error event of the ML$^D$ decoder that is resulted from three or more errors in the two channel outputs is upper bounded by $O(p^3)$. In addition, if at least one of the channel's outputs is of length exactly $n$, then this channel output is the transmitted codeword and hence a unique and correct decoding is guaranteed.  Therefore, a decoding error of probability $o(p^3)$ can occur only in the case where there is exactly one error in each channel output. 
Let $\bfy_1$ and $\bfy_2$ be the channel outputs, such that $\bfy_1$ is obtained from $\bfx$ by deleting one symbol from the $i$-th run of the transmitted word $\bfx$, and $\bfy_2$ is obtained by deleting one symbol from the $j$-th run of $\bfx$. W.l.o.g. assume $i \le j$, and consider the following three cases. \\ 
\textbf{Case 1:} If $i=j$ by Lemma~\ref{lm:2ch_run_del}, there is a decoding error with probability of $\prun(q,\hspace{-0.25ex}p) \hspace{-0.3ex}$.
\\ \textbf{Case 2:} If $i \ne j$ and for each $i<\ell<j$ (if exists), the length of the $\ell$-th run of the transmitted word $\bfx$ is 1, then the subsequence of consecutive symbols between the right most index of the $i$-th run of $\bfx$ and the left most index of the $j$-th run of $\bfx$ is an alternating sequence. Therefore, by Lemma~\ref{lm:2ch_alt_del}, there is a decoding error with probability of $\palt(q,\hspace{-0.25ex}p) \hspace{-0.3ex}$. 
\\ \textbf{Case 3:} Otherwise, we have that $i \ne j$ and there exists  $i<\ell<j$, such that the $\ell$-th run of the transmitted word $\bfx$ is of length at least $2$. It can be verified that in this case $d_H(\bfy_1, \bfy_2)>1$.  Hence, by Proposition 9, that was proved in~\cite{ISIT20}, there is a unique and correct decoding if and only if $\bfy_1$ and $\bfy_2$ are not \emph{Type-A confusable}, where the definition of  Type-A confusable is as follows. We say that two words, $\bfy_1$ and $\bfy_2$ are Type-A confusable if there exist $\bfa$, $\bfb$, $\bfc$, such that $\bfy_1= \bfa \bfc \bfb$, $\bfy_2=\bfa \bar{\bfc} \bfb$, where $\bar{\bfc}$ is the complement of $\bfc$ and either $\bfc = (\alpha \beta)^m$ or $(\alpha \beta)^m\beta$ for some $m>0$ and $\alpha, \beta \in \Sigma_q$. We denote by $h_i$ and $h_j$ the index of the right most, left most symbol of the $i$-th, $j$-th run, respectively.  It can be readily verified that $\bfy_1$ and $\bfy_2$ are equal up to the $(h_i-1)$-th index, and hence $\bfa = \bfx_{[1:h_i-1]}$. Similarly, these two words have the same suffix $\bfb = \bfx_{[h_j+1:n]}$. Let $\bfc$, such that $\bfy_1 = \bfa \bfc \bfb$, note that the latter implies that the $\ell$-th run of $\bfx$ is within the word $\bfc$, which implies that $\bfc$ is not an alternating sequence. Additionally, the last run in $\bfc$ consists only from the first symbol of the $j$-th run of $\bfx$ and hence $\bfc$ cannot be of the form $\bfc=(\alpha \beta)^m \beta$. Thus, $\bfy_1$ and $\bfy_2$ are not Type-A confusable, which guarantees a unique and correct decoding. That is the error probability of the ML$^D$ decoder in this case equals zero.}
\end{comment}
\begin{comment}
 from the Lemma's assumption, it is known that the deletion of the $i$-th symbol of $\bfy_1$ and the deletion of the $i+j$-th symbol of  $\bfy_2$ are deletions from two different runs of the transmitted word.  
The proof follows from the above few lemmas. Note that each run error translates to an increase of the Levenshtein distance by one. On each occurrence of the alternating event the decoder chooses the correct subsequence with probability 0.5 and every error increases the Levenshtein distance by two since it translates to one insertion and one deletion. Lastly, the $O(p^3)$ expression compensates for all other less dominant error events which introduce more than two deletions that are close to each other at least in one of the channels.
\end{comment}
\begin{comment}
We consider the following possible error events.
\begin{enumerate}
\item There is a deletion in the $i$-th index of both channels. In this case there is also a deletion in the output of ${ML}^*$ decoder. The Levenshtein error probability of this event is $p^2$.
\item There are deletions in indices $i$ and $i+1$ in the two channels, which happens in probability $2p^2$. If $\bfx_{[i,i+1]}$ is a run then there is a deletion in the output of the ${ML}^*$ decoder. This event happens with probability $1/q$. If $\bfx_{[i,i+1]}$ is an alternating sequence, then the ${ML}^*$ output is correct with probability 1/2 or output a sequence of Levenshtein distance 2 with probability 1/2. This event happens with probability $(q-1)/q$. Hence, the Levenshtein error probability of this event is 
$$2p^2\left(1\cdot \frac{1}{q} +\frac{1}{2}\cdot 2\cdot \frac{q-1}{q} \right)= 2p^2.$$
\item There are deletions in indices $i$ and $i+2$ in the two channels, which happens in probability $2p^2$. If $\bfx_{[i,i+2]}$ is a run then there is a deletion in the output of the ${ML}^*$ decoder. This event happens with probability $(1/q)^2$. If $\bfx_{[i,i+2]}$ is an alternating sequence, then the ${ML}^*$ output is correct with probability 1/2 or output a sequence of Levenshtein distance 2 with probability 1/2. This event happens with probability $(q-1)/q^2$. Hence, the Levenshtein error probability of this event is 
$$2p^2\left(1\cdot \frac{1}{q^2} +\frac{1}{2}\cdot 2\cdot \frac{q-1}{q^2} \right)= \frac{2p^2}{q}.$$
%\item There are deletions in indices $i$ and $i+3$ in the two channels, which happens in probability $2p^2$. If $\bfx_{[i,i+3]}$ is a run then there is a deletion in the output of the ML decoder. This event happens with probability $(1/q)^3$. If $\bfx_{[i,i+3]}$ is an alternating sequence, then the ML output is correct with probability 1/2 or output a sequence of Levenshtein distance 2 with probability 1/2. This event happens with probability $(q-1)/q^3$. Hence, the Levenshtein error probability of this event is  $$2p^2\left(1\cdot \frac{1}{q^3} +\frac{1}{2}\cdot 2\cdot \frac{q-1}{q^3} \right)= \frac{2p^2}{q^2}.$$
\item There are deletions in indices $i$ and $i+c$ in the two channels, which happens in probability $2p^2$. If $\bfx_{[i,i+c]}$ is a run then there is a deletion in the output of the ${ML}^*$ decoder. This event happens with probability $(1/q)^c$. If $\bfx_{[i,i+c]}$ is an alternating sequence, then the ${ML}^*$ output is correct with probability 1/2 or output a sequence of Levenshtein distance 2 with probability 1/2. This event happens with probability $(q-1)/q^c$. Hence, the Levenshtein error probability of this event is 
$$2p^2\left(1\cdot \frac{1}{q^c} +\frac{1}{2}\cdot 2\cdot \frac{q-1}{q^c} \right)= \frac{2p^2}{q^{c-1}}.$$
\end{enumerate}
\e{Note that the Levenshtein error rate, as well as the success rate of the ${ML}^*$, are also affected by deletions of two (or more) symbols in $\bfx_{[i,i+1]}$. The probability and the Levenshtein error rate this case are O($p^3$).}

Together, we receive the Levenshtein error rate is
$$p^2 + 2p^2\sum_{c=1}^{\infty}\frac{1}{q^{c-1}} = p^2 +\frac{2q}{q-1}p^2 = 2p^2+\frac{q+1}{q-1}p^2 + O(p^3).$$
\end{IEEEproof}
\end{comment}

Using these observations, we are also able to approximate the average decoding failure probability. 
\begin{theorem}\label{th:2chF}
The average decoding failure probability is 
$$\pfail(q,p) \gtrsim  e^{-\frac{3q-1}{q-1}p^2n}.$$
\end{theorem} 
\begin{IEEEproof}
This probability is bounded from below by the probability that there was neither a deletion error because of the runs nor errors because of the alternating sequences. 
Hence, a lower bound on this probability is 
\begin{align*} 
 \left( 1- \prun(q,p) \right)^n \cdot \left( 1- \palt(q,p) \right)^n  \approx  \left( 1- (\prun(q,p) +  \palt(q,p)) \right)^n =  \left( 1-\frac{3q-1}{q-1}p^2 \right)^n  \approx e^{-\frac{3q-1}{q-1}p^2n}.& \end{align*}  %\\[-2.5\baselineskip] 
 \end{IEEEproof} 

So far we have discussed only the case in which the code $\cC$ is the entire space. However, the most popular deletion-correcting code is the VT code~\cite{VT}. Recently, SVT, an extension of the VT code, has been proposed in~\cite{7837631} for the correction of burst deletions. The goal of the SVT code is to correct a deletion error while its position is known up to some roughly $\log(n)$ consecutive locations. However, this construction has been recently used in~\cite{8294216} to build a code that is specifically targeted for the reconstruction of a word that is transmitted through two single-deletion channels. 
Due to the relevance of correcting deletion and alternating errors, the decoding failure probabilities of these two codes are investigated in this work. We abbreviate the notation of $\pfail(\del(p),2,VT_n,\cD_{\ML^D}), \pfail(\del(p),2,SVT_n,\cD_{\ML^D})$ by $\pfail(VT_n,q,p),\pfail(SVT_n,q,p)$, respectively. The following theorem summarizes these results. 
\begin{theorem}\label{th:2ch_VT}
The average decoding failure probabilities for the VT and SVT codes are given by
\begin{small}
\begin{align*}
\pfail(VT_n,q,p)  &\gtrsim  \left( 1- \prun(q,p) \right)^n \cdot \left( 1- \palt(q,p) \right)^n  & \\
& + \left( 1- \prun(q,p) \right)^{n} \cdot n \palt(q,p) \left( 1- \palt(q,p) \right)^{n-1} & \\
& + n \prun(q,p)\left( 1- \prun(q,p) \right)^{n-1} \cdot \left( 1- \palt(q,p) \right)^{n}, & \\
\pfail(SVT_n,q,p)  &\gtrsim  \left( 1- \prun(q,p) \right)^n \cdot \left( 1- \palt(q,p) \right)^n  & \\
& + \left( 1- \prun(q,p) \right)^{n} \cdot n \palt(q,p) \left( 1- \palt(q,p) \right)^{n-1}.& 
\end{align*}
\end{small}
\end{theorem}
\begin{IEEEproof}
The proof follows from the observation that the VT code is capable of decoding either a single run error or a single alternating error. On the other hand, the shifted VT code is capable of only correcting a single alternating error; see~\cite{8294216} for more details. 
\end{IEEEproof}

We verified the theoretical results presented in this section by computer simulations. These simulations were performed over words of length $n=450$ which were used to create two noisy copies given a fixed deletion probability $p\in[0.005,0.05]$. Then, the two copies were decoded by the ML$^D$ decoder as described earlier in this section. Finally, we calculated the Levenshtein error rate of the decoded word as well as its average decoding failure probability (referred to here as \emph{failure rate}). Fig.~\ref{fig:LER-Deletion} plots the results of the Levenshtein error rate, which is the average Levenshtein distance between the decoder's output and the transmitted simulated word, normalized by the transmitted word's length. This value evaluates the expected normalized distance. Fig.~\ref{fig:LER-Deletion} confirms the approximation of the probability  $\perr(q,p)$. Similarly, in Fig.~\ref{fig:runAltErrorsDel} we present the error probabilities $\palt(q,p)$ and  $\prun(q,p)$ separately, along with the corresponding value as calculated in Lemma~\ref{lm:2ch_run_del},~\ref{lm:2ch_alt_del}, respectively. Lastly, in Fig.~\ref{fig:failuerRate}, we simulated the ML$^D$ decoder for the VT codes and the SVT codes and calculated the failure rate $\pfail(q,p)$. The implementation of the VT code was taken from~\cite{DBLP:journals/corr/abs-1906-07887}, and we modified this implementation for SVT codes. 
		\begin{figure}[h!]
		\centering
		\subfigure{\includegraphics[width=85mm]{plots/LER-Del.png}}
		\caption{The Levenshtein error rate as a function of the deletion probability $p$. The Levenshtein error rate is the average Levenshtein distance between the decoder's output and the transmitted simulated word, normalized by the transmitted word's length.  This value is an approximation of the expected normalized distance. } %These simulations verify Theorem~\ref{th:2ch}.}
		 \label{fig:LER-Deletion}
	\end{figure}
	\begin{figure}[h!] 
		\centering
		\subfigure{\includegraphics[width=85mm]{plots/runAltErrors.png}}
		\caption{The Levenshtein error rate as a function of the deletion probability $p$. These simulations verify Lemma~\ref{lm:2ch_run_del} and Lemma~\ref{lm:2ch_alt_del}.}\label{fig:runAltErrorsDel}
	\end{figure}


	\begin{figure}[h!] 
		\centering
		\subfigure{\includegraphics[width=85mm]{plots/FailureRateColor.png}}
		\caption{Failure rate of the ML$^D$ decoder, stratified by the coding scheme. These simulations verify Theorem~\ref{th:2chF} and Theorem~\ref{th:2ch_VT}.}\label{fig:failuerRate}
	\end{figure}

%We demonstrated and verified the results of Theorem~\ref{th:2ch} by simulations: In each simulation we took a random word of size n, created two noisy copies (traces) of this word given a fixed deletion probability p, and decode this traces with the $ML^*$ decoder. Then, we calculated the Levenshtein error rate of the decoded word (compare to the transmitted word). For each deletion probability we made 200,000 simulations and calculate the average LER. The results of these simulations are presented in Figure~\ref{fig:LER-Deletion} 



%In Theorem~\ref{th:2ch}, we can interpret $\frac{q+1}{q-1}p^2$ to be the deletion error rate that results from the deletions in the runs and $2p^2$ is the LER that results from mis-decoding because of the alternating sequences. These results are also verified in the following simulation we ran. We analyzed both the deletion probability and the LER. To do so, we partitioned the outputs of the ML decoder into sets, based upon the length. We presented separately the LER for tests with decoded words of size n (we interpret those words as having LER caused by alternating sequences) and the LER for decoded words of any size (these words includes Levenshtein errors cause by alternating and runs). These results, as well as the bounds from Theorem~\ref{th:2ch} are presented in~Figure~\ref{fig:LER-Deletion-RUNALT}.%We analyzed both the deletion probability and the LER. To do so, we partitioned the outputs of the ML decoder into sets, based upon the length. For any length, we expected the LER to be fixed and equal $2p^2$. That implies also that the size of the ML SCS should be roughly $2p^2n$.

\begin{comment}

    \begin{minipage}[t]{\linewidth}
        \includegraphics[width = 1\textwidth]{plots/LER-Deletion-RUNALT.png}
         \captionof{figure}{Levenshtein error rate by the deletion probability. In this simulation the parameters were: the length of the tested words was 450, the alphabet size was 4 and the number of simulation for each deletion probability is 200,000}
        \label{fig:LER-Deletion-RUNALT}
    \end{minipage} 
 \footnote{\e{Omer, here we need to put simulation results for two deletions and support all of these results. We need to think how to do it.}}

\end{comment}
\begin{comment}
\subsection{Two Deletions Using the Varshamov Tenengolts Codes}

$P_{success}=(1-p_{run})^n(1-p_{alt})^n + (1-p_{run})^{n}(1-p_{alt})^{(n-1)}np_{alt}+
(1-p_{run})^{(n-1)}n(p_{run})(1-p_{alt})^{n}$


$P_{run}=\frac{q+1}{q-1}p^2 = 3p^2$

$P_{alt}=p^2 = p^2$


\subsection{Two Deletions Using the Shifted Varshamov Tenengolts Codes}
$P_{success}=(1-p_{run})^n(1-p_{alt})^n + (1-p_{run})^{n}(1-p_{alt})^{(n-1)}np_{alt}$


$P_{run}=\frac{q+1}{q-1}p^2 = 3p^2$

$P_{alt}=2*0.5*p^2 = p^2$
\end{comment}



Complexity wise, it is well known that the time complexity to calculate the SCS length and the embedding numbers of two sequences are both quadratic with the sequences' lengths. However, the number of SCSs can grow exponentially~\cite{itoga1981string, elzinga2008algorithms}.  Thus, given a set of SCSs of size $L$, the complexity of the ML$^D$ decoder for $t=2$ will be $O(Ln^2)$. The main idea behind these algorithms uses dynamic programming in order to calculate the SCS length and the embedding numbers for all prefixes of the given words. However, when calculating for example the SCS for $\bfy_1$ and $\bfy_2$ it is already known that $\mathsf{SCS}(\bfy_1,\bfy_2) \leq n$. Hence, it is not hard to observe that (see e.g.~\cite{apostolico1992fast}) many paths corresponding to prefixes which their length difference is greater than $d_1+d_2$ can be eliminated, when $d_1,d_2$ is the number of deletions in $\bfy_1,\bfy_2$, respectively. In particular, when $d_1$ and $d_2$ are fixed, then the time complexity is linear. In our simulations we used this improvement when implementing the ML$^D$ decoder. Other improvements and algorithms of the ML decoder are discussed in~\cite{srinivasavaradhan2018maximum,srinivasavaradhan2019symbolwise}.




\section{Two Insertion Channels}\label{sec:ins}
%\input{1-insertion}
This section continues the two-channel study but for the insertion case. In a similar manner to the deletion case, the ML$^D$ decoder is defined as 
\begin{align*}
 \cD_{\ML^D}(\bfy_1, \bfy_2) \triangleq \argmin_{\bfx\in \subs(\bfy_1, \bfy_2)} \left\{ \emb(\bfx ; \bfy_1) \emb(\bfx ; \bfy_2)\right\}. 
\end{align*}
This section proves that, similarly to the deletion case, the dominant errors resulting from increasing the length of a run in both of the channel outputs and error that results from the occurrence of an alternating sequence. We denote by $\perrin(q,p)$ the approximated expected normalized distance of the ML$^D$ decoder upon two instances of the insertion channel $\ins(p)$. Similarly, $\pfailin(q,p)$ is the average decoding failure probability and lastly 
$\prunin(q,p), \paltin(q,p)$ is the insertion probability due to runs, occurrence probability due to alternating sequences, respectively. The following theorem summarizes the results of this section. 
\begin{theorem}\label{th:ins}
For the insertion channel $\ins(p)$, it holds that 
\begin{align*}
& \prunin(q,p) \approx \frac{q+1}{q(q-1)}p^2, \ %\\ \text{and} \\&
\paltin(q,p)  \approx \frac{2}{q}p^2.\\
%& \perrin(q,p) \approx \frac{3q-1}{q(q-1)}p^2 + O(p^3), \ \  \pfailin(q,p) \approx e^{-\frac{2}{q-1}p^2n}.
\end{align*}
\end{theorem}

The proof of this theorem repeats the same ideas as the ones for the deletion case. However, we list here the relevant lemmas and their proofs for the completeness of the results in this section. \vspace{-2ex}
\begin{comment}
\begin{theorem}\label{th:ins}
For the insertion channel $\ins(p)$, it holds that \vspace{-.5ex}
\begin{align*}
& \prunin(q,p) \approx \frac{q+1}{q(q-1)}p^2, \ \ \ \paltin(q,p)  \approx \frac{2}{q}p^2, \\
& \perrin(q,p) \approx \frac{3q-1}{q(q-1)}p^2 + O(p^3). % \ \  \textcolor{red}{\pfailin(q,p) \approx e^{-\frac{2}{q-1}p^2n}}.
\end{align*}
\end{theorem}
\textcolor{red}{The proof of this theorem repeats the same ideas as the ones for the deletion case. We summarize here the relevant lemmas and their proofs. }
\end{comment}
 \begin{lemma} \label{lm:2ch_run_ins}
For the insertion channel $\ins(p)$, it holds that 
%It holds that The average deletion probability of the ML decoder's output because of the runs is at least 
$$\prunin(q,p)  \approx \frac{q+1}{q(q-1)}p^2.$$
\end{lemma}\vspace{-1ex} 
\begin{IEEEproof} 
The probability that both channels have experienced an insertion in a given run of length $r$ is roughly ${((r+1)\cdot \frac{p}{q})^2}$. Similarly to our proof of Lemma~\ref{lm:2ch_run_del}, the occurrence probability of a run of length exactly $r$ is $\frac{q-1}{q} \cdot \left(\frac{1}{q}\right)^{r-1}  $. Thus, for $n$ large enough, the error probability is approximated by 
%\begin{small}
\begin{align*}
\sum_{r=0}^{\infty} \left((r+1)\cdot\frac{p}{q}\right)^2  \frac{q-1}{q} \cdot \left(\frac{1}{q}\right)^{r-1}  &= \frac{p^2}{q^2}\cdot \frac{q-1}{q} \sum_{r=0}^{\infty} (r+1)^2 \left(\frac{1}{q}\right)^{r-1} & \\
& = \frac{p^2}{q^2}\cdot \frac{q-1}{q} \cdot \frac{q^3(q+1)}{(q-1)^3} = p^2\cdot \frac{(q+1)}{(q-1)^2}.& 
\end{align*}
%\end{small}
%The expected length of a run is given by 
%$$\sum_{r=1}^{\infty} r \left(\frac{1}{q}\right)^{r-1}\cdot\frac{q-1}{q} =\frac{q-1}{q} \sum_{r=1}^{\infty} r \left(\frac{1}{q}\right)^{r-1} = \frac{q}{q-1}.$$
The expected number of runs in a vector of length $n$ is $n\cdot \frac{q-1}{q}$, and thus the approximated number of insertions to the decoder output due to runs is 
$$n\cdot \frac{q-1}{q} \cdot p^2\cdot \frac{(q+1)}{(q-1)^2}= n p^2\cdot  \frac{q+1}{q(q-1)},$$
which verifies the statement in the lemma. \end{IEEEproof}


\begin{lemma} \label{lm:2ch_alt_ins}
For the insertion channel $\ins(p)$, it holds that 
%It holds that The average deletion probability of the ML decoder's output because of the runs is at least 
$$\paltin(q,p)  \approx \frac{2}{q}p^2.$$
\end{lemma} \vspace{-1ex}
\begin{IEEEproof}
%Given two insertions, one in the first channel in the $i$-th position, and the second is in the second channel in the $i+j$-th position (or $i-j$-th position)
Assume there are two close insertions. The first insertion is in the $i$-th position of the first channel, and the closest insertion in the second channel is in position $i+j$. If $\bfx_{[i:i+j]}$ is an alternating sequence $ABAB\cdots$, the same output from the two channels could be received if the transmitted word is the same as $\bfx$ but with the opposite order for the symbols of the alternating sequence, that is, the symbols of the word in the positions of $[i:i+j]$ are $BABA\cdots$. The same holds if the closest insertion in the second channel is in position $i-j$.
Therefore, the occurrence probability of this event can be approximated by
$$2(\frac{p}{q})^2\cdot \sum_{j=0}^\infty \frac{q-1}{q}\cdot \frac{1}{q^{j-1}} = \frac{2}{q}\cdot p^2,$$
where  $\frac{q-1}{q}\cdot \frac{1}{q^{j-1}}$ is the probability that $\bfx_{[i:i+j]}$ is any alternating sequence and the multiplication by 2 takes into account the cases of deletion in either position $i-j$ or $i+j$.
\end{IEEEproof}

Similarly to our discussion in Section~\ref{sec:two deletions}, it should be noted that the approximations that were calculated in Lemma~\ref{lm:2ch_run_ins} and in Lemma~\ref{lm:2ch_alt_ins}, are in fact upper bounds of $\prunin(q,p) $ and $\paltin(q,p)$ in our simulations. Hence the Levenshtein error rate for two insertion channels is approximated by 
$$\perrin(q,p) \lesssim \prunin(q,p) + \paltin(q,p) +O(p^3) = \frac{3q-1}{q(q-1)}p^2+O(p^3).$$

\begin{comment}
\begin{lemma} 
If there is an insertion in the first, second channel in position $i-1, i+j$, where $j>0$, respectively, and the sequence $\bfx_{[i:i+j]}$ is neither a run nor an alternating sequence, then these insertions are corrected successfully by the ML decoder. 
%If there are deletions in positions $i$ and $i+c$ for $c\geq 1$, and the transmitted word is of the shape of $x=(\bfx_{[0:i-1},\bfx_{[i:i+c]}, \bfx_{[i+c+1,n]}$, where $\bfx_{[i:i+c]}$ is not the alternating sequence or a run, then the ${ML}^*$ decoder can successfully decode the word $x$. 
\end{lemma}
%\begin{comment}
\begin{IEEEproof}
\e{The output of the first channel is $(A, x_i, x_{i+1},x_{i+2},\ldots,x_{i+j})$ and the one of the second channel is $(x_{i},x_{i+1},\ldots,x_{i+j}, B)$. Clearly, it holds that $(x_i,x_{i+1},x_{i+2},\ldots,x_{i+j})$ is a candidate for the ML$^D$ decoder. Let the vector $\widehat{\bfx}'=(x_i',x_{i+1}',x_{i+2}',\ldots,x_{i+j}')$ be another candidate for the ML$^D$ decoder. The insertions occurred in positions $i-1$ and $i+j$. Hence, adding $A'$ to the $i$ position of  $\widehat{\bfx}'$ or $B'$ to its $i+j+1$ position will result as the two channels. Hence, it should hold that $$(A', x_i',x_{i+1}',x_{i+2}',x_{i+3}',\ldots,x_{i+j}') =$$ $$(x_{i}, x_{i+1},x_{i+2}, x_{i+3},\ldots , x_{i+j-2} ,x_{i+j-1} ,x_{i+j}, B)$$
and  
$$(x_{i}',x_{i+1}',x_{i+2}',x_{i+3}', \ldots,x_{i+j}', B') =$$ $$(A, x_i, x_{i+1},x_{i+2}, x_{i+3}, \ldots, x_{i+j-2},  x_{i+j-1},x_{i+j}).$$
Therefore we get that $x_i=x_{i+2}=x_{i+4}=\cdots $ and $x_{i+1}=x_{i+3}=x_{i+5}=\cdots $, i.e., $\bfx_{[i:i+j]}$ is either the alternating sequence or a run, which results with a contradiction.}
\end{IEEEproof}
\begin{theorem}\label{th:ins}
The Levenshtein error rate for two insertion channels is approximated by 
\vspace{-1.5ex} $$\hspace{-0.3ex}\perrin(q,\hspace{-0.25ex}p)\hspace{-0.35ex} \approx\hspace{-0.35ex} \prunin(q,\hspace{-0.25ex}p) \hspace{-0.3ex}+\hspace{-0.3ex} \paltin(q,\hspace{-0.25ex}p) \hspace{-0.3ex}+\hspace{-0.3ex}O(p^3) \hspace{-0.3ex}=\hspace{-0.3ex} \frac{3q\hspace{-0.3ex}-\hspace{-0.3ex}1}{q(q\hspace{-0.3ex}-\hspace{-0.3ex}1)}p^2\hspace{-0.3ex}+\hspace{-0.3ex}O(p^3).$$
\end{theorem} \vspace{-1.5ex}
\begin{IEEEproof}
The proof follows from the above few lemmas. Note that each run error translates to an increase of the Levenshtein distance by one. On each occurrence of the alternating event the decoder chooses the correct subsequence with probability 0.5 and every error increases the Levenshtein distance by two since it translates to one insertion and one deletion. Lastly, the $O(p^3)$ expression compensates for all other less dominant error events which introduce more than two deletions that are close to each other at least in one of the channels.
\end{IEEEproof}
\end{comment}


The theoretical results of Theorem~\ref{th:ins} have also been verified by simulation results over words of length $n=500$, which were used to create two noisy copies with a given fixed insertion probability $p\in[0.005,0.05]$. Then, the two copies were decoded with the ML$^D$ decoder. Lastly, we calculated and plotted in Fig.~\ref{fig:LER-Insertion} the Levenshtein error rate as well as the error rates from runs and alternating sequences.% along with the corresponding expression of $\perrin(q,p)$. 
\begin{figure}[h!] 
		\centering
		\subfigure{\includegraphics[width=85mm]{plots/LER-Ins.png}}
		\caption{The Levenshtein error rate as a function of the insertion probability $p$. This simulation verifies Theorem~\ref{th:ins}. }\label{fig:LER-Insertion}
	\end{figure}
\begin{comment}	
    \begin{minipage}[t]{\linewidth}
        \includegraphics[width = 1\textwidth]{plots/LER-Ins.png}
         \captionof{figure}{Levenshtein error rate by the insertion probability $p$. This simulation verifies Theorem~\ref{th:ins}.  In this simulation the parameters were: the length of the tested words was $n=500$, the alphabet size $q=2$ and the number of simulation for each deletion probability $p$ is 1,000,000}
        \label{fig:LER-Insertion}
    \end{minipage}   
\end{comment}


==> Intersection/abstract.tex <==
This paper studies the intersections of insertion and deletion balls. The $t$-insertion, $t$-deletion ball of a sequence $\bfx$ is the set of all sequences received by $t$  insertions, deletions to $\bfx$, respectively. While the intersection of either deletion balls or insertion balls has been rigorously studied before, the intersection of an insertion ball and a deletion ball has not been addressed so far. We find the maximum intersection size of any two insertion and deletion balls in the binary case. For the special case of one-insertion and one-deletion balls we find the intersection size for all pair of sequences. Then, we derive the largest and average values of this intersection size. Lastly, we present an algorithm that efficiently computes the intersection of any $t_1$-insertion ball and $t_2$-deletion ball.

==> Intersection/algo.tex <==
\label{sec:alg}
In this section, we address Problem~\ref{prob4} and present an efficient algorithm that given $y_1\in \Sigma^{n-t_1}_2$, $y_2\in \Sigma^{n+t_2}_2$, and $n$ calculates $|\ID(\bfy_1,\bfy_2,n)|$. A naive method to calculate this intersection is to compute these two balls, i.e., $I_{t_1}(\bfy_1)$ and $D_{t_2}(\bfy_2)$, and then calculate their intersection. However, since the calculation of the balls is done recursively, this approach will introduce high complexity\footnote{since the size of $I_{n-|\bfy_1|}(\bfy_1)$ is $\Theta(|\bfy_1|^{n-|\bfy_1|})$ and the largest size of $D_{|\bfy_2|-n}(\bfy_2)$ is $\Theta(|\bfy_2|^{|\bfy_2|-n})$, the worst case complexity of this solution is $\Theta(n^{|\bfy_2|-|\bfy_1|+1})= \Theta(n^{t_1+t_2+1})$.}. The algorithm described in this section is based on dynamic programming, and hence works more efficiently. %For shorthand, we abbreviate the intersection $I_{n-|\bfy_1|}(\bfy_1) \cap D_{|\bfy_2|-n}(\bfy_2)$ by $\ID(\bfy_1,\bfy_2,n)$.
%While in the previous cases of only insertions and only deletions, we could use existing algorithms for finding the SCS and LCS, here it is necessary to  find the intersection of an insertion ball and a deletion ball. A naive solution is to calculate these two balls, i.e., $I_{n-|\bfy_1|}(\bfy_1)$ and $D_{|\bfy_2|-n}(\bfy_2)$, and then calculate their intersection. However, this approach will introduce high complexity\footnote{since the size of $I_{n-|\bfy_1|}(\bfy_1)$ is $\Theta(|\bfy_1|^{n-|\bfy_1|})$ and the largest size of $D_{|\bfy_2|-n}(\bfy_2)$ is $\Theta(|\bfy_2|^{|\bfy_2|-n})$, the worst case complexity of this solution is $\Theta(n^{|\bfy_2|-|\bfy_1|+1})$.}, and hence we show next how to operate this procedure more efficiently. For shorthand, we abbreviate the intersection $I_{n-|\bfy_1|}(\bfy_1) \cap D_{|\bfy_2|-n}(\bfy_2)$ by $\ID(\bfy_1,\bfy_2,n)$. 

The following additional definitions will be used throughout the section. A sequence $\bfx$ is called a \emph{common subsequence} of some words $\bfy_1,\ldots,\bfy_t$ if $\bfx$ is a subsequence of each one of these $t$ words. The set of all common subsequences of $\bfy_1,\dots,\bfy_t$ is denoted by  $\cC\cS(\bfy_1,\ldots,\bfy_t)$ and
 $\mathsf{LCS}(\bfy_1,\dots,\bfy_t)$ denotes the \emph{length of the longest common subsequence} (\emph{LCS)} of $\bfy_1,\dots,\bfy_t$, that is, $\mathsf{LCS}(\bfy_1,\dots,\bfy_t) = \max_{\bfx\in \cC\cS(\bfy_1,\ldots,\bfy_t)}\{|\bfx|\}$. The set of all longest common subsequences of $\bfy_1,\dots,\bfy_t$ is denoted by  $\subs(\bfy_1,\ldots,\bfy_t)$.


\begin{comment}
Given \EY{$\bfy_1\in \del(p,x)$, $\bfy_2\in \ins(p,x)$} and $n\in\mathbb{N}$ the decoder goal is to calculate
\begin{align*}
\bfx' & = \argmax_{\bfx\in\{0,1\}^n}\left\{ \emb(\bfx;\bfy_1)\cdot \emb(\bfy_2;\bfx) \right\} & \\ 
& =  \argmax_{\bfx\in C(\bfy_1,\bfy_2,n)}\left\{ \emb(\bfx;\bfy_1)\cdot \emb(\bfy_2;\bfx) \right\}, & 
\end{align*}
where $C(\bfy_1,\bfy_2,n)$ is the intersection of $\Sigma_2^n$  and the support of \EY{$\emb(\bfx;\bfy_1)\cdot \emb(\bfy_2;\bfx)$}.

Hence, a generic algorithm for the decoder can be defined as follows,
\begin{algorithm}
  \caption{Maximum Likelihood Decoder}
  \begin{algorithmic}
   \State Input: $y_1, y_2, n$
   \State Calculate $C(y_1,y_2,n)$ 
   \State max = 0
   \For {each $x\in C(y_1,y_2,n)$}
    \State likelihood = Emb($x;y_1$)$\cdot$ Emb($y_2;x$)
    \If{likelihood $\ge$ max}
    \State max = likelihood
    \State curr = x
    \EndIf
    \EndFor
    \State Return curr
  \end{algorithmic}
\end{algorithm}\\

Let $T_{\mathsf{Emb}}$ and $T_{C}$ be the average time complexities of calculating the expression $\emb(\cdot; y_1)\cdot \emb(y_2;\cdot)$ and the set $C(y_1,y_2,n)$ respectively. Then the average time complexity of the above algorithm is $\theta\left(T_C + |C(y_1,y_2,n)|\cdot T_{Emb}\right)$.

\section{Calculating $C(y_1,y_2,n)$}

\begin{observation}
Let $\bfx$ be a sequence. Then $\bfx\in C(\bfy_1,\bfy_2,n)$ if and only if $\bfx\in\Sigma^n$, $\bfy_1$ is a subsequence of $\bfx$ and $\bfx$ is a subsequence of $y_2$.  
\end{observation}
\end{comment}

Let us denote by $\mathcal{U}(\bfy_1,\bfy_2)$ the set of index sets $U$ such that the projection of $\bfy_2$ on the index set $U$ yields $\bfy_1$, that is,
\[
\mathcal{U}(\bfy_1,\bfy_2) = \left\{U\subseteq [|\bfy_2|]:\ (\bfy_2)_U = \bfy_1\right\}.
\]
%For an index set $I$, define its \emph{indices vector}, denoted by $\bfv_I$, to be the vector which consists of all the indices in $I$ in an increasing order. We say that $I$ is a \emph{right-most index set of $\bfy$}, if there is no other index set $I'$ such that $\bfy_I=\bfy_{I'}$ and \e{$\bfv_{I'}\geq \bfv_I$}. Furthermore, denote by $\mathcal{I}_{right}(\bfy_1,\bfy_2)\subseteq \mathcal{I}(\bfy_1,\bfy_2)$ the set of all right-most index sets of $\bfy_2$. \textcolor{red}{Say something about canonical embeddings}. We next show how to exhaustively and efficiently scan all vectors in the set $\ID(\bfy_1,\bfy_2,n)$. This will be done by first considering the right-most index sets of $\bfy_2$ that their projection yields $\bfy_1$ and then complete them with an arbitrary set of indices on the remaining set of indices to receive a length-$n$ word in $\ID(\bfy_1,\bfy_2,n)$.
We say that an index set $U$ is a \emph{right-most index set} of a sequence $\bfy$ if all the indices of $U$ are the right most indices in their run in $\bfy$, i.e., for all $i\in U$, either $i$ is the right most index of its run in $\bfy$, or $i+1\in U$.  Furthermore, denote by  $\mathcal{U}_{right}(\bfy_1,\bfy_2)\subseteq \mathcal{U}(\bfy_1,\bfy_2)$ the set of all right-most index sets of $\bfy_2$ in $\mathcal{U}(\bfy_1,\bfy_2)$\footnote{Not to be confused with the right canonical embedding (also called canonical embedding) presented in~\cite{E08}. The right canonical embedding is defined as the embedding that consists of the largest possible indices, and note that the canonical embedding is unique.}.
We next show how to exhaustively and efficiently~\footnote{It is possible to show that the expectation of $|\mathcal{U}_{right}|$ is upper bounded by $O(n^{\min \{t_1, t_2 \}})$. Therefore, for fixed values of $t_1$ and $t_2$, the average time complexity of Algorithm~\ref{alg1} is $O(n^{\min \{t_1, t_2 \}})$. } scan all vectors in the set $\ID(\bfy_1,\bfy_2,n)$. This will be done by first considering the right-most index sets of $\bfy_2$ such that the corresponding projections yields $\bfy_1$ and then complete them with an arbitrary set of indices on the remaining set of indices to receive a length-$n$ word in $\ID(\bfy_1,\bfy_2,n)$.
\begin{theorem}~\label{the:C}
It holds that \vspace{-.7ex}
\begin{small}
\begin{align*} 
&\ID(\bfy_1,\bfy_2,n) & \\
&= \left\{(\bfy_2)_{U\cup V}\hspace{-.3ex}:\hspace{-.3ex} U \in\mathcal{U}_{right}(\bfy_1,\bfy_2), V\subseteq\left[|\bfy_2|\right]\backslash U,\ |V|=n-|U| \right\}. &
\end{align*}
\end{small}
\end{theorem}
%\begin{lemma}\label{lem:if}
%Let $I\in\mathcal{I}_{right}(\bfy_1,\bfy_2)$  and $J\subseteq\left[|\bfy_2|\right]\backslash I$ be an index set such that $|J| = n - |I|$, then $(\bfy_2)_{I\cup J}\in \ID(\bfy_1,\bfy_2,n)$. 
%\end{lemma}
\begin{IEEEproof}
Let $U\in\mathcal{U}_{right}(\bfy_1,\bfy_2)$. By definition, $(\bfy_2)_U=\bfy_1$. Hence, $\bfy_1$ is a subsequence of $(\bfy_2)_{U\cup V}$. In addition, since $U\cup V\subseteq \left[|\bfy_2|\right]$, $\bfy_2$ is a supersequence of $(\bfy_2)_{U\cup V}$. That is, $\bfy_2$ can be obtained from $(\bfy_2)_{U\cup V}$  by $|\bfy_2|-|U\cap V|$ insertions and  $\bfy_1$ can be obtained from $(\bfy_2)_{U\cup V}$ by $|V|$ deletions. Namely, that is to say that  $(\bfy_2)_{U\cup V}\in\ID(\bfy_1,\bfy_2,n)$.

For the other direction, let $\bfx\in\ID(\bfy_1,\bfy_2,n)$ be a sequence. By definition, $\bfx$ is a subsequence of $\bfy_2$. Hence, there is a set of indices $T\subseteq\left[|\bfy_2|\right]$ such that $(\bfy_2)_T=\bfx$. Let the number of indices in $T$ that are contained in the $i$-th run of $\bfy_2$ be denoted by $T(i)$ and let $T'$ be the index set that consists of the $T(i)$ right-most indices of the $i$-th run of $\bfy_2$ for $1\le i\le r(\bfy_2)$. Then. it holds that $(\bfy_2)_{T'}=\bfx$.
In addition, since $\bfy_1$ is a subsequence of $\bfx=(\bfy_2)_{T'}$, there is a set of indices $U\subseteq T'$ such that $(\bfy_2)_U = \bfy_1$. Since the indices in $T'$ are the right-most indices of each run of $\bfy_2$, there is an index set $U'\subseteq T'$ that consists of the $U(i)$ right-most indices of the $i$-th run of $\bfy_2$ for $1\le i\le \rho(\bfy_2)$ and satisfies $(\bfy_2)_{U'}=\bfy_1$. That is, $U'\in\mathcal{U}_{right}(\bfy_1,\bfy_2)$ and for $V=T'\backslash U'$ we have that $(\bfy_2)_{U'\cup V} = (\bfy_2)_{T'}=\bfx$.
\end{IEEEproof}
%\begin{IEEEproof} \DB{add proof} \end{IEEEproof}

Using Theorem~\ref{the:C} we have the following algorithm for the calculation of the intersection $\ID(\bfy_1,\bfy_2,n)$,\vspace{-1ex}
\begin{algorithm}
  \caption{$\ID(\bfy_1,\bfy_2,n)$}  \label{alg:1}
  \begin{algorithmic}
   \State Input: $\bfy_1, \bfy_2, n$
   \State Calculate $\mathcal{U}_{right}(\bfy_1,\bfy_2)$ 
  \State Set $S=\emptyset$
    \For {each $U\in\mathcal{U}_{right}(\bfy_1,\bfy_2)$}
    \For {each $V\subseteq\left[|\bfy_2|\right]\backslash U$ such that $|V|=n-|U|$}
    \State  Calculate $\bfx=(\bfy_2)_{U\cup V}$
    \State Set $S=S\cup\{\bfx\}$
    \EndFor
    \EndFor
    \State Return $S$
  \end{algorithmic}\label{alg1}
\end{algorithm}%\vspace{-1ex}

 Notice that replacing any index in $j\in V$ with an index $j'\in \left[|\bfy_2|\right]\backslash \left(U\cup V\right)$ from the same run of $\bfy_2$ has no affect on $(\bfy_2)_{U\cup V}$. That is, $(\bfy_2)_{U\cup V} = (\bfy_2)_{U\cup (V\backslash\{j\})\cup {j'}}$ for any two indices $j,j'\notin U$ such that $j\in V, j'\notin V$ and $j,j'$ belong to the same run in $\bfy_2$. Hence, in the second for loop of Algorithm~\ref{alg1}, it is sufficient to iterate only over indices sets $V$ that differ in the number of indices from the same run.
 
It is left to calculate the sets of index sets $\mathcal{U}_{right}(\bfy_1,\bfy_2)$. The algorithm to calculate $\mathcal{U}_{right}(\bfy_1,\bfy_2)$ is based on the dynamic programming implementation of the LCS problem~\cite{I81}, which is shortly explained next. Given two words $\bfx,\bfy$, let $\mathsf{LCS}(i,j)$ denote the length of the LCS of $\bfx_{[i]}$ and ${\bfy}_{[j]}$. The length of the LCS of $\bfx$ and $\bfy$ is given by $\mathsf{LCS}(|\bfx|,|\bfy|)$ and is computed using the following recursive formula

\vspace{-2ex}
\begin{small}
$$\mathsf{LCS}(i,j) =\begin{cases}   0 & i=0 \text{ or } j=0\\ 1+\mathsf{LCS} (i-1,j-1)  & \bfx(i) = \bfy(j) \\ \max \{ \mathsf{LCS}(i-1,j) , \mathsf{LCS}(i, j-1) \} & \text{otherwise} \end{cases}$$
\end{small}
\noindent The implementation of this computation is done using a $(|\bfx|+1) \times( |\bfy|+1) $ matrix, which is referred as the \emph{dynamic programming table}, where the $j$-th entry of the $i$-th row of the dynamic programming table quals to $\mathsf{LCS}(i,j)$. 

%The dynamic programming implementation is done using the recursive formula $$\mathsf{LCS}(i,j) =\begin{cases}   0 & i=0 \text{ or } j=0\\ 1+LCS (i-1,j-1)  & \bfx_1(i) = \bfx_2(j) \\ \max \{ LCS(i-1,j) , LCS(i, j-1) \} & \text{otherwise} \end{cases}$$ where $LCS(i,j)$ denotes the length of the LCS of two sequences ${\bfx_1}_{[i]}$ and ${\bfx_2}_{[j]}$, i.e $\mathsf{LCS}({\bfx_1}_{[i]}, {\bfx_2}_{[j]})$. That is, the length of LCS of $\bfx_1$ and $\bfx_2$ is given by $LCS(|\bfx_1|,|\bfx_2|)$. 
The calculation of the set of index sets in $\mathcal{U}_{right}(\bfy_1,\bfy_2)$ will also be done using the $(|\bfy_1|+1) \times( |\bfy_2|+1) $ dynamic programming table. Observe that under the problem specifications, $\bfy_1$ is a subsequence of $\bfy_2$, and thus it holds that $\mathcal{LCS}(\bfy_1,\bfy_2) = \{\bfy_1\}$ and thus $\mathsf{LCS}(|\bfy_1|,|\bfy_2|) = |\bfy_1|$. Therefore, there exists at least one index set $U$ such that $(\bfy_2)_U=\bfy_1$.  However, in order to find all such right-most index sets, the idea is to search within the dynamic programming table, in order to identify these index sets $U$ which consist of only the right-most indices of each run of $\bfy_2$ and satisfy $(\bfy_2)_U=\bfy_1$.

In order to search such index sets $U$ within the dynamic programming table in an efficient way, we use some of its properties. First, note that the size of each such set $U$ is $|\bfy_1|$. Let $U = \{ i_1, i_2, \ldots, i_{|\bfy_1|} \}$, since $({\bfy_2})_U = \bfy_1$, the $j$-th entry of the $i_j$-th column of the dynamic programming table equals to $j$. By the above, the column that corresponds to the $i_j$-th index contains the value $j$ in the $j$-th entry, and the $i_j$-th index represents the appearance of the $j$-th symbol of $\bfy_1$ in $\bfy_2$. 
Since each selected index $i_j$ corresponds to the $j$-th symbol of $\bfy_1$, which corresponds to the $j$-th row of the dynamic programming table, the selection of $i_j$ allows us to eliminate the $j$-th row of the dynamic programming table from the rest of the search. We choose the indices of $U$ in a backward order, and by doing so each selection of index reduces the number of rows by one in the matrix we need to search in the rest of the algorithm. %one row from the matrix we need to search at at the rest of the search.   the $|y_1|$-th row of the dynamic programming table to its first row.  %Furthermore, when traversing the $i$th row, in order to be able to assemble $\bfy_1$, it holds that the value at the entry $(i,j)$ is not smaller than $i$.  In fact, the entry value can not be greater than $i$ since all the entries at $i$th row are bounded by $i$ from above.

Before we present the explicit algorithm to compute the set  $\mathcal{U}_{right}(\bfy_1,\bfy_2)$, let us introduce a few data structures that will be used in the algorithm.
\begin{enumerate}
    \item A two-dimensional array, called $\mathsf{match}$, such that {${\mathsf{match}(i,j)=1}$} if $\bfy_1[i]=\bfy_2[j]$ and otherwise $0$.
    \item A two-dimensional array $\mathsf{LCS}$, which is the dynamic programming table of the LCS algorithm. 
    \item A binary vector $\mathsf{curr}$ of length $|\bfy_2|$. The set of non-zero entries of $\mathsf{curr}$ correspond to the indices in a set $U\in \mathcal{U}_{right}(\bfy_1,\bfy_2)$ in the current step of the search.  
   \end{enumerate}
By using the above characterization, we design the following recursive procedure, presented in Algorithm~\ref{alg:C}, in order to calculate the set $\mathcal{U}_{right}(\bfy_1,\bfy_2)$. Algorithm~\ref{alg:C} is initially invoked with the sequences $\bfy_1$ and $\bfy_2$, the indices $i=|\bfy_1|,\ j=|\bfy_2|$, and the all zero vector $\mathsf{curr}$.
\begin{algorithm}
  \caption{The calculation of $\mathcal{U}_{right}$}
  \begin{algorithmic}
   \State \textbf{Input:}  $\bfy_1$, $\bfy_2$, $i$, $j$ and a pointer to $\mathsf{curr}$
%   \State {}
    \State $\mathcal{U}_{right}=\emptyset$.
   \If {$i=0$ or $j=0$}
   \State  $\mathcal{U}_{right} \leftarrow \{\mathsf{curr}\} \cup \mathcal{U}_{right}$
   \State Return $\mathcal{U}_{right}$
   \EndIf
   \If{$\mathsf{LCS}(i,j)<i$}
   \State Return $\mathcal{U}_{right}$ 
   \EndIf
    \If{$\mathsf{match}(i,j) = 1$ and $(j=n$ or $\bfy_2[j] \neq \bfy_2[j-1]$ or $\mathsf{curr}[j] = 1)$}
    \State Set $\mathsf{curr}[j-1] \leftarrow 1$
    \State $\mathcal{U}_{right} \leftarrow \mathcal{U}_{right} \cup \text{Algorithm 2}(\mathsf{curr}, \bfy_1, \bfy_2, i-1, j-1)$ 
    \State Set $\mathsf{curr}[j-1] \leftarrow 0$
    \EndIf
\If{$\mathsf{LCS}(i,j-1)=i$}
    \State $\mathcal{U}_{right} \leftarrow \mathcal{U}_{right} \cup \text{Algorithm 2}(\mathsf{curr}, \bfy_1, \bfy_2, i, j-1)$ 
\EndIf
\State Return $\mathcal{U}_{right}$. \vspace{-1.5ex}
  \end{algorithmic}~\label{alg:C} %\vspace{-1.5ex}
\end{algorithm} %\vspace{-2ex}

The next example demonstrates the idea of Algorithm~\ref{alg:C}. 

%\vspace{3ex}
\begin{example}
Consider the example shown in Fig.~\ref{fig:alg_ex}, in which $\bfy_1=0010$ and $\bfy_2=000111010$ and each table is the dynamic programming table. The four highlighted columns in each table correspond to one set of indices $U\in\mathcal{U}_{right}$.

\begin{figure}[h!] 
\centering
%\vspace{1ex}
\subfigure{\includegraphics[width=.728\linewidth]{plots/example.png}} \vspace{-1ex}
\caption{An example of Algorithm~\ref{alg:C} for $\bfy_1=0010$ and $\bfy_2=000111010$, so $\mathsf{LCS}(\bfy_1, \bfy_2)=4$. The highlighted columns represent the right-most index sets $U \in \mathcal{U}_{right}(\bfy_1,\bfy_2)$. More specifically, theses sets, ordered in a clockwise manner, are: $ \{3,7,8,9 \}, \{2,3,6,9 \}, \{ 2,3,8,9\}, \{2,3,6,7\} $. }\label{fig:alg_ex} \vspace{-2ex}
\end{figure}
\end{example}

\begin{theorem} 
Let $\bfy_1$ and $\bfy_2$ be two sequences such that $|\bfy_1|\le |\bfy_2|$. The output of Algorithm~\ref{alg:C} is $\mathcal{U}_{right}(\bfy_1,\bfy_2)$ if $\bfy_1$ is a subsequence of $\bfy_2$, and is $\emptyset$ otherwise.
\end{theorem}
\vspace{-.7ex}
\begin{IEEEproof} Let $\mathcal{U}_{right}$ denote the output of Algorithm~\ref{alg:C} for an input of $\bfy_1$ and $\bfy_2$, i.e.,
$$\mathcal{U}_{right}=\text{Algorithm~\ref{alg:C}}(\mathsf{curr},\bfy_1,\bfy_2,\abs{\bfy_1},\abs{\bfy_2}).$$

If $\bfy_1$ is not a subsequence of $\bfy_2$ it must be that $1\le \abs{\bfy_1}$, and by the assumption, $\abs{\bfy_1}\le \abs{\bfy_2}$. 
Thus, the first if condition does not hold. Also, it must be that $\mathsf{LCS}(\abs{\bfy_1},\abs{\bfy_2})< \abs{\bfy_1}$, so the algorithm output is $\mathcal{U}_{right}=\emptyset$.

Let us assume that $\bfy_1$ is a subsequence of $\bfy_2$. 
First, we will prove that $\mathcal{U}_{right}\subseteq\mathcal{U}_{right}(\bfy_1,\bfy_2)$. 
At the initialization $i\le j$ and in each recursive call we can decrease both $i$ and $j$ by one or only decrease $j$ by one. 
Since the latter is possible only if $i = \mathsf{LCS}(i,j-1)\le \min\{i,j-1\} \le j-1$, it holds that $i\le j$ throughout the run of the algorithm. 
For convenience, we consider the vector $\mathsf{curr}$ to be the index set $U:=\{j\ |\ \mathsf{curr}[j-1]=1\}$ it represents.  
An index set $U$ is inserted to $\mathcal{U}_{right}$ only when the first if condition holds, that is, only if $i=0$ or $j=0$ and since $i\le j$, that is, whenever $i=0$. By the definition of the algorithm, $i$ and $U$ can only be changed when the third if condition holds. 
In this case, $j$ is inserted to $U$ and $i$ and $j$ are decreased by one.  
Thus, if $i=0$, $U$ must contain $|\bfy_1|$ indices $j_1,\ldots, j_{\abs{\bfy_1}}$ and by the third condition each $j_i$ satisfies $(\bfy_1)_i=(\bfy_2)_{j_i}$. 
Therefore, each index set $U$ in the output  satisfies $\bfy_1=(\bfy_2)_{U}$ which implies  that $\mathcal{U}_{right}\subseteq\mathcal{U}(\bfy_1,\bfy_2)$. 

Let $U\in\mathcal{U}_{rignt}$, and denote by $j_1<j_2<\cdots <j_{\abs{\bfy_1}}$ the indices in $U$. 
Since $(\bfy_2)_U=\bfy_1$,  for $1\le i\le \abs{\bfy_1}$ it holds that $(\bfy_2)_{\{ j_i, \ldots, j_{\abs{\bfy_1}} \}}=(\bfy_1)_{[i\ :\ \abs{\bfy_1}]}$.
 We will prove, by backward induction that $\{ j_1, \ldots, j_{\abs{\bfy_1}}\}$ is a right-most index set.
For $i=\abs{\bfy_1}$, if $j_{\abs{\bfy_1}}=\abs{\bfy_2}$ it is clearly a right-most index set. 
Otherwise, due to the fact that $j_{\abs{\bfy_1}}$ was inserted into $U$ in the third if condition of the algorithm,  it must be that $(\bfy_2)_{j_{\abs{\bfy_1}}}\ne (\bfy_2)_{j_{\abs{\bfy_1}}+1}$ (it can not be that $j_{\abs{\bfy_1}}+1\in U$ since $U$ is empty). 
Thus, $j_{\abs{\bfy_1}}$ is the right-most index in its run in ${\bfy_2}$ and $\{ j_{\abs{\bfy_1}} \}$ is a right-most index set. Let us assume that $\{ j_{i+1}, \ldots ,j_{\abs{\bfy_1}} \}$ is a right-most index. 
Similarly to the base case,  $j_i$ was inserted into $U$ in the third if condition. 
Hence, it must be that $(\bfy_2)_{j_i}\ne(\bfy_2)_{j_i+1}$ or that $j_i+1\in U'$ where $U'$ is the subset of $U$ in the current step of the algorithm.  
By the induction assumption $\{ j_{i+1}, \ldots, j_{\abs{\bfy_1}} \}$ is a right-most index set and if $(\bfy_2)_{j_{i}}\ne(\bfy_2)_{j_i+1}$, then $j_i$ is the right-most index in its run and  $\{ j_i, j_{i+1},\ldots,j_{\abs{\bfy_1}} \}$ is also a right-most index set. 
Otherwise, $j_i$ and $j_{i}+1$ belong to the same run of $\bfy_2$ and $j_i+1\in U'$.   
By the induction assumption all the indices that are greater than $j_i+1$ and belong to the same run as $j_i+1$ are also in $U'$, that is, all the indices that are right to $j_i$ and at the same run are in $U'$ and  $\{j_i, j_{i+1},\ldots,j_{\abs{\bfy_1}}\}$ is a right-most index set by definition. 
We have proven that each index set $U\in\mathcal{U}_{right}$ is a right-most index set, that is, we have proven that $\mathcal{U}_{right}\subseteq \mathcal{U}_{right}(\bfy_1,\bfy_2)$.

To see that $\mathcal{U}_{right}(\bfy_1,\bfy_2)\subseteq \mathcal{U}_{right}$ consider some index set $U\in \mathcal{U}_{right}(\bfy_1,\bfy_2)$ and let $j_1<\cdots< j_{\abs{\bfy_1}}$ be the indices in $U$. 
Since $U\in\mathcal{U}_{right}(\bfy_1,\bfy_2)$, for each $i$ and $j\ge j_i$ we have that $\mathsf{LCS}(i,j)=i$, that is, the fourth condition holds. Consider the path that invokes the first recursive call  if and only if $j=j_i$ for some index $1\le i\le \abs{\bfy_1}$, and invokes the second recursive call otherwise.  Since $U$ is a right-most index set, one can easily verify that this is a valid path of the algorithm that yields the index set $U$ and append it to the algorithm output $U_{right}$. 
\end{IEEEproof}

%\section{Performance Evaluation}
We used simulations to evaluate the performance of Algorithm~\ref{alg:1}.  Our simulations worked on 4 different values of $n=\{50, 75, 100, 125\}$. For each $n$, we created $5,000$ test cases as follows. First, the values of $t_1$ and $t_2$ were generated according to the standard normal distribution with mean $\mu =4$ and standard deviation of $\sigma=0.5$. Next, $\bfy_2$ was selected randomly from all the sequences of length $n+t_2$. Then, $t_2+t_1$ bits were selected randomly and deleted from $\bfy_2$ to create $\bfy_1$. We then performed Algorithm~\ref{alg:1} and the naive algorithm (described in the begining of this section) to compute $\ID(\bfy_1, \bfy_2, n)$ and evaluated their run time. Both algorithms were implemented in $c++$ and performed on our server with Intel(R) Xeon(R) CPU E5-2630 v3 2.40GHz. In all of the tests Algorithm~\ref{alg:1} performed the computation of $\ID(\bfy_1, \bfy_2, n)$ significantly faster and improve the speed of the naive algorithm by a factor of more than $5,000$. The results of the tests are summarized in Table~\ref{tab:res}.  Note that we performed the comparison over relatively small values of the parameters due to the limitations of the naive algorithm.   
\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c| } 
 \hline
 $n$ & The Naive Algorithm & Algorithm~\ref{alg:1} \\
 \hline
 50 & 1558 & 6.37 \\ 
 75 & 10449 & 6.79 \\ 
 100 & 44652 & 8.38 \\ 
 125 & $>88000$ & 9.46 \\ 
 \hline

\end{tabular}
\end{center}
 \caption{A comparison of the run time (in seconds) of Algorithm~\ref{alg:1} and the naive algorithm to compute $\ID(\bfy_1, \bfy_2, n)$.} \label{tab:res}
\end{table}

==> Intersection/intro.tex <==
Studying the size of the deletion and insertion balls as well as their intersections is the one of the more intriguing combinatorial problems in the area of coding for synchronization channels. The $t$-deletion ball of some sequence $\bfx$ is defined to be the set of all sequences that can be derived from $\bfx$ by exactly $t$ deletions. Similarly the $t$-insertion ball of $\bfx$ is the set of all words that can be received by $t$ insertions to $\bfx$.  While it is well known that the insertion balls are regular, that is, the ball size does not depend on the center word $\bfx$, the deletion balls sizes indeed depend on the center $\bfx$~\cite{L65}. In particular, the minimum size of the deletion ball is achieved when $\bfx$ consists of a single symbol, while the maximum size is received only for the alternating words. 

Studying~\cite{GY18,L01B,SGSD17} the intersection of deletion and insertion balls has several applications. For example, the largest size of these intersections provide the solution for the sequence reconstruction problem, which was first studied by Levenshtein~\cite{L01A,L01B}, for insertion and deletion channels. These largest sizes correspond to the required minimum number of channels when transmitting a codeword over several deletion or insertion channels. These problems have also connection to the generalized Gilbert-Varshamov bound~\cite{JV04}, associative memories~\cite{JLL19,YB18}, and list decoding~\cite{JY18,LTX19,W17}. One of the motivations to specifically study the intersection of a deletion ball together with an insertion ball originates from a recent problem we addressed in~\cite{SYY20}. Assume a sequence $\bfx$ is transmitted over two channels, where the first introduces deletions while the second only insertions. In order to find the list of all possible transmitted sequences, it is necessary to find the intersection of the insertion ball of the first channel's output and the deletion ball of the second channel's output. While significant progress has been accomplished in studying the intersections of either deletion balls or insertion balls, to the best of our knowledge there is no study that considers together the intersection of insertion and deletion balls of two arbitrary words, which is the goal of this paper. Lastly, we note that studying the intersection of insertion and deletion balls contributes also to studying the balls in the Levenshtein metric and the intersection of these balls~\cite{BEY21,SaDo13,SGD14}. 

The rest of the paper is organized as follows. Section~\ref{sec:gen_comb} presents the definitions used throughout the paper, a necessary and sufficient condition for the intersection of an insertion ball and a deletion ball to be nonempty, and the problems that will be solved in the paper. In Section~\ref{sec:max} we study the maximum size of a $t_1$-insertion ball and  a $t_2$-deletion ball for the binary case. Section~\ref{sec:1int} addresses the case of one-insertion and one-deletion balls. We find the intersection size for all words $\bfy_1$ and $\bfy_2$ such that $\bfy_1$ is a subsequence of $\bfy_2$. Based on this result we also derive the largest intersection size and the average size of this intersection. Lastly, in Section~\ref{sec:alg} we present an efficient algorithm to compute the intersection of two insertion and deletion balls. It is shown how to improve upon a naive solution, which computes first the deletion and insertion balls of the two sequences and then find their intersection. Due to the lack of space, some of the proofs in the paper are omitted.

==> Intersection/maxinter.tex <==
In this section, we fully solve Problem~\ref{prob1} for the binary case, i.e., the case where $\bfy_1\in\Sigma_2^{n_1}$ and $\bfy_2\in\Sigma_2^{n_2}$.  

\begin{theorem}\label{th:max}
For integers $0\le t_1\le n$, $0 \le t_2$,  and $q=2$ we have that \vspace{-3ex}
$$\max_{\substack{\bfy_1\in \Sigma_2^{n-t_1}, \bfy_2\in\Sigma_2^{n+t_2}}}|\ID(\bfy_1,\bfy_2,n)| = \sum_{i=0}^{\min\{t_1, t_2\}}\binom{n}{i}.$$
\end{theorem}
\begin{IEEEproof}
Let $\bfy_1\in\Sigma_q^{n-t_1},\bfy_2\in\Sigma_q^{n+t_2}$. If $t_1 \ge t_2$,  we have that \vspace{-2ex}
$$|\ID(\bfy_1,\bfy_2,n)| \hspace{-0.25ex}=\hspace{-0.25ex} |I_{t_1}(\bfy_1)\cap D_{t_2}(\bfy_2)|\hspace{-0.25ex}\le\hspace{-0.25ex} |D_{t_2}(\bfy_2)| \hspace{-0.25ex}\le\hspace{-0.25ex} \sum_{i=0}^{t_2}\binom{n}{i},\vspace{-0.75ex}$$
where the last inequality is proven in~\cite{H99, L65}. To see that the upper bound is tight, let $\bfy_2$ be an alternating segment of length $n+t_2$ and let $\bfy_1$ be the word that is obtained by deleting the last $t_1+t_2$ symbols of $\bfy_2$. Note that $\bfy_1$ is an alternating segment of length $n-t_1$. By~\cite{H99}, $|D_{t_2}(\bfy_2)|= \sum_{i=0}^{t_2}\binom{n}{i}$. In addition, any deletion in any word can decrease the number of runs by at most $2$. Hence, for each $\bfx\in D_{t_2}(\bfy_2)$, $\rho(\bfx)\ge n+t_2 - (t_1+t_2) = n-t_1$. Note that if the first symbol of $\bfx$ and $\bfy_2$ is different, then the latter inequality is strong. In this case it is possible to show that we can delete $t_1$ more bits in $\bfx$ %(one has to distinguish between the cases whether $\bfx$ and $\bfy_1$ start with the same bit) 
in order to receive $\bfy_1$, that is, $\bfx$ is a supersequence of $\bfy_1$ and hence $\bfx\in \ID(\bfy_1,\bfy_2,n)$, which implies that $|\ID(\bfy_1,\bfy_2,n)| = \sum_{i=0}^{t_2}\binom{n}{i}$.

The case $t_1 < t_2$ is proved in a similar way using the insertion ball of $\bfy_1$ in order to upper bound the size of $\ID(\bfy_1,\bfy_2,n)$  (the size of the insertion ball is given in~\cite{L65}).

%For the case where $t_1 < t_2$, we can use the insertion ball of $\bfy_1$ in order to upper bound the size of $|\ID(\bfy_1,\bfy_2,n)|$, that is, $$|\ID(\bfy_1,\bfy_2,n)| = |I_{t_1}(\bfy_1)\cap D_{t_2}(\bfy_2)|\le |I_{t_1}(\bfy_1)|= \sum_{i=0}^{t_1}\binom{n}{i}.$$ To see that this bound is tight, we consider the alternating words $\bfy_1$ and $\bfy_2$ from the previous case. The following strategy explains how $\bfy_2$ can be obtained by inserting $t_2$ symbols to any word $\bfx \in I_{t_1} (\bfy_1)$.   Recalll that $\bfy_1$ is the alternating word of length $n-t_1$, and any word  $\bfx \in I_{t_1} (\bfy_1)$ is obtained from $\bfy_1$ by inserting $t_1$ symbols. Given any order on the inserted symbols, we denote by $\sigma_i$ the $i$-th inserted symbol. By replacing each of these insertions by an insertion of two different symbols $\sigma_i \sigma_i' $ (or $\sigma_i' \sigma_i$), such that $\sigma_i \ne \sigma_i'$, we get the alternating word of length $n+t_1$. Lastly, by concatinating to this word the alternating sequence of length $t_2-t_1$, the word $\bfy_2$ is obtained. 
\end{IEEEproof}

==> Intersection/prelem.tex <==
\label{sec:gen_comb}
%In this section we present the definitions and notations that will be used throughout the paper.
Let $\Sigma_q$ denote the set of integers $\{0,1,\ldots,q-1\}$ and for an integer $n\ge0$,
let $\Sigma_q^n$ be the set of all sequences (words) of length $n$ over the alphabet $\Sigma_q$. For a word $\bfx\in\Sigma_q^*$, let $|\bfx|$ denote the length of $\bfx$.
For an integer $t$, $0\le t\le n$, a sequence $\bfy\in\Sigma_q^{n-t}$ is a \emph{$t$-subsequence} of
$\bfx\in\Sigma_q^n$ if $\bfy$ can be obtained from $\bfx$ by deleting $t$ symbols from $\bfx$.
That is, there exist $n-t$ indices $1\le i_1<i_2<\cdots<i_{n-t}\le n$ such that $y_j=x_{i_j}$, for all $1\le j\le n-t$. We say that $\bfy$ is a \emph{subsequence} of $\bfx$ if $\bfy$ is a $t$-subsequence of $\bfx$ for some $t$.
Similarly, a sequence $\bfy\in\Sigma_q^{n+t}$ is a \emph{$t$-supersequence} of
$\bfx\in\Sigma_q^n$ if $\bfx$ is a $t$-subsequence of~$\bfy$.

For a sequence $\bfx\in\Sigma_q^n$, let $\bfx_{[i,j]}$ be the subsequence $x_ix_{i+1}\cdots x_{j}$ and for a set of indices  $U\subseteq \{1,\ldots,n\}$, the sequence ${\bfx}_{U}$ is the \emph{projection} of $\bfx$ on the indices of $U$, which is the subsequence of $\bfx$ received by the symbols in the entries of $U$. 
%For a symbol ${\sigma\in \Z_q}$, $\sigma^n$ denotes the sequence with $n$ consecutive $\sigma$'s.
%The \emph{Hamming weight} of a word $\bfx\in\Sigma_q^n$ is denoted by $\wt{\bfx}$ and is equal to the number of nonzero coordinates in $\bfx$. The \emph{Hamming distance} between two words ${\bfx,\bfy\in\Sigma_q^n}$, denoted by $d_H(\bfx,\bfy)$, is the number of coordinates in which $\bfx$ and $\bfy$ differ.
For  $\bfx,\bfy\in\Sigma_q^*$, the \emph{Levenshtein distance} between $\bfx$ and $\bfy$, $d_L(\bfx,\bfy)$,
is the smallest number of insertions and deletions that is required to transform $\bfx$ into $\bfy$.\vspace{-0.5ex}
\begin{definition}
The {\emph{\bf $\bft$-deletion ball}} centred at ${\bfx\in\Sigma_q^n}$, $D_t(\bfx)\subseteq \Sigma_q^{n-t}$, is the set of all $t$-subsequences of~$\bfx$.
%\end{definition}
%\begin{definition}
The {\emph{\bf $\bft$-insertion ball}} centred at ${\bfx\in\Sigma_q^n}$, $I_t(\bfx)\subseteq \Sigma_q^{n+t}$, is the set of all $t$-supersequences of $\bfx$.
\end{definition}\vspace{-0.5ex}


For a sequence $\bfx\in\Sigma_q^n$,
a \emph{run} of $\bfx$ is a maximal subsequence $\bfx_{[i,j]}$ of identical symbols. The number of runs in $\bfx$ is denoted by $\rho(\bfx)$.
We say that $\bfx_{[i,j]}$ is an \emph{alternating segment}
if $\bfx_{[i,j]}$ is a sequence of alternating distinct symbols $\sigma,\sigma'\in \Sigma_q$.
Note that $\bfx_{[i,j]}$ is a \emph{maximal alternating segment} if $\bfx_{[i,j]}$ is an alternating segment
and $\bfx_{[i-1,j]},\bfx_{[i,j+1]}$ are not. For example, for $\bfx=00110121$,  $\rho(\bfx) = 6$ and the four maximal alternating segments are $0$, $01$, $101$, $121$. 

%\section{Problem Statement}
In this work we study \emph{the insertion-deletion intersection problem}. In this problem we let $\bfy_1, \bfy_2 \in \Sigma_q^*$ and $n\in\N$ such that $|\bfy_1|\le n\le |\bfy_2|$ and the goal is to find the set of all words $\bfx\in\Sigma_q^n$ such that $\bfx$ is both,  a supersequence of $\bfy_1$ and a subsequences of $\bfy_2$. That is, to find the set\vspace{-1ex}
\[
\ID(\bfy_1,\bfy_2,n)\triangleq I_{n-|\bfy_1|}(\bfy_1) \cap D_{|\bfy_2|-n}(\bfy_2).\vspace{-1ex}
\]
The following lemma states a necessary and sufficient condition for $\ID(\bfy_1,\bfy_2,n)=\emptyset$.

\begin{lemma}
\label{lem: iff cond.}
%Let  $\bfy_1,\bfy_2 \in \Sigma_q^*$, and let $n$ be an integer such that $|\bfy_1|\le n\le |\bfy_2|$, then $d_L(\bfy_1, \bfy_2) > |\bfy_2|-|\bfy_1|$  if and only if $\ID(\bfy_1,\bfy_2,n) = {\emptyset} $.
Let  $\bfy_1,\bfy_2 \in \Sigma_q^*$, and let $n$ be an integer such that $|\bfy_1|\le n\le |\bfy_2|$.
Then, $\ID(\bfy_1,\bfy_2,n) \neq {\emptyset}$ if and only if $\bfy_1$ is a subsequence of $\bfy_2$. 
\end{lemma}
\begin{IEEEproof}
Let $\delta \triangleq |\bfy_2|-|\bfy_1|$. Since $|\bfy_1|\le |\bfy_2|$, we must perform at least $\delta$ insertions in order to transform $\bfy_1$ into $\bfy_2$, and hence $d_L(\bfy_1,\bfy_2)\ge\delta$.
Assume $d_L(\bfy_1,\bfy_2)= \delta$ then $\bfy_1$ is obtained by deleting $\delta$ symbols from $\bfy_2$. That is, there exists a set of indices $U\subseteq[|\bfy_2|]$ such that $|U|=\delta$ and
$(\bfy_2)_{[|\bfy_2|]\backslash U} = \bfy_1.$
Let $U'\subseteq U$ be a set of indices such that $|U'| = |\bfy_2|-n$.
It can be easily verified that\vspace{-1ex} $$ (\bfy_2)_{[|\bfy_2|]\backslash U'}\in \ID(\bfy_1,\bfy_2,n)\vspace{-1ex}$$ and hence,
$
\ID(\bfy_1,\bfy_2,n) \ne {\emptyset}. 
$ 

For the other direction, assume $d_L(\bfy_1,\bfy_2)>\delta$ and assume to the contrary that there exists $\bfx\in\Sigma_q^n$ such that 
$\bfx\in \ID(\bfy_1,\bfy_2,n)$. In this case, $\bfx$ can be obtained from $\bfy_2$ by $|\bfy_2|-n$ deletions and $\bfy_1$ can be obtained from $\bfx$ by $n-|\bfy_1|$ deletions, which is a contradiction since $d_L(\bfy_1,\bfy_2)>\delta$.
%Since $\bfx\in D_{|\bfy_2|-n}(\bfy_2)$, $\bfx$ is a subsequence of $\bfy_2$ and $\bfx$ can be obtained from $\bfy_2$ by $|\bfy_2|-n$ deletions. Similarly, since $\bfx\in I_{n-|\bfy_1|}(\bfy_1)$, $\bfy_1$ is a subsequence of $\bfx$ and $\bfy_1$ can be obtained from $\bfx$ by $n-|\bfy_1|$ deletions. 
%Therefore, $\bfy_1$ can be obtained from $\bfy_2$ by $|\bfy_2|-n+n-|\bfy_1|=\delta$ deletions which is a contradiction since $d_L(\bfy_1,\bfy_2)>\delta$.
\end{IEEEproof}  

According to Lemma~\ref{lem: iff cond.}, it is assumed in the rest of the paper that $\bfy_1$ is a subsequence of $\bfy_2$. 
The goal of this paper is to study the following problems.
\begin{problem}\label{prob1}
Given integers $n_1\le n\le n_2$, find the maximum intersection size, i.e., 
 $\max_{\substack{\bfy_1\in \Sigma_q^{n_1}, \bfy_2\in\Sigma_q^{n_2}}}|\ID(\bfy_1,\bfy_2,n)|$. 
\end{problem}
\begin{problem}\label{prob2}
Given integers $n_1\le n\le n_2$, find the expected intersection size for only nonempty intersections, %\vspace{-0.5ex}
$$\mathop{{}\mathbb{E}}_{\substack{\bfy_1\in \Sigma_q^{n_1}, \bfy_2\in\Sigma_q^{n_2}\\ \bfy_1 \text{ is a subsequence of } \bfy_2}}\left[|\ID(\bfy_1,\bfy_2,n)|\right].$$%\vspace{-1ex}$$
\end{problem}
\begin{problem}\label{prob3}
Given $\bfy_1,\bfy_2\in\Sigma_q^*$ and an integer $n$ such that $|\bfy_1|\le n\le |\bfy_2|$, find the size of $\ID(\bfy_1,\bfy_2,n)$. 
\end{problem}
\begin{problem}\label{prob4}
Given $\bfy_1,\bfy_2\in\Sigma_q^*$ and an integer $n$ such that $|\bfy_1|\le n\le |\bfy_2|$, find efficient algorithms to calculate the set $\ID(\bfy_1,\bfy_2,n)$. 
\end{problem}

\begin{comment}
The goal of this section is to study the intersection or radius-one 
Note that if $|\bfy_1| = n-1$ and $|\bfy_2| = n+1$ then $d_L(\bfy_1, \bfy_2) \ge 2$. 

From this point it is assumed that  $d_L(\bfy_1, \bfy_2) = 2$.
Let $\bfy \in \Sigma_q^n$ be a word of length $n$ such that $\rho(\bfy)=k$. The run-length profile vector of $\bfy$, denoted by $\widehat{r}(\bfy)$, is a $2 \times k$ matrix that satisfies the following rules. 
\begin{enumerate}
\item For $1\le i \le k$, the value of the $i$-th entry of the first row is $\sigma_i \in \Sigma_q$, which is the symbol of the $i$-th run of $\bfy$. 
\item For  $1\le i \le k$, the value of the $i$-th entry of the second row is $r_i$, which is the length of the $i$-th run of $\bfy$.
\end{enumerate}

For example, if $\bfy = 111001010000$, then $\rho(\bfy) = k = 6$, and 
$$ \widehat{r}(\bfy)=
\begin{bmatrix}
1 & 0 & 1 & 0 & 1 & 0\\
3 & 2 & 1 & 1& 1 & 4
\end{bmatrix}
$$
Note that the summation of the values of the entries in the second row of $\widehat{r}(\bfy)$ equals to the length of $\bfy$.
\end{comment}

\begin{comment}
Further note that any insertion to $\bfy$ can either create new run, or prolong an existing run. 
Denote by $\bfx$, a word that obtained from $\bfy$ by inserting one symbol. If the insertion prolongs the $i$-th run of $\bfy$, the number of runs in $\bfx$ equals $\rho(\bfx)=\rho(\bfy) =k$, and the run-length profile of $\bfx$ differs from the one of $\bfy$ by exactly one entry. The difference reflects the length of $i$-th run of $\bfx$, which its length equals $r_i+1$. Otherwise, if the insertion creates a new run, there are two distinct cases.
\begin{enumerate}
\item The new run is added before the first run of $\bfy$ (or after the last run of $\bfy$). In this case, the number of runs in $\bfx$ is $\rho(\bfx) = \rho(\bfy)+1=k+1$, and the run length profile of $\bfx$ differs from the one of $\bfy$ by only having one additional column in the beginning (in the end). In our example $\bfx = 0111001010000$, and 
$$ \widehat{r}(\bfx)=
\begin{bmatrix}
0 & 1 & 0 & 1 & 0 & 1 & 0\\
1 & 3 & 2 & 1 & 1& 1 & 4
\end{bmatrix}.
$$
\end{comment}

\begin{comment}
\item The new run is added within the i-th run of $\bfy$, for $i=k$ (or alternatively $i=1$). In this case, the number of runs in $\bfx$ is $\rho(\bfx) = \rho(\bfy)+1=k+2$, and the run length profile of $\bfx$ is exactly the same as the one of $\bfy$ up to the $k$-th column (or up to the $k$-th column from the end), then the $k$-th run (or $k$-th run from the end) has length $s$ from some $s<r_k$, the $k+1$-th run has length $1$, and the last run has length $r_k-s$ In our example for $s=1$, $\bfx = 1110010101000$, and 
$$ \widehat{r}(\bfx)=
\begin{bmatrix}
1 & 0 & 1 & 0 & 1 & 0 & 1 &0\\
3 & 2 & 1 & 1& 1 & 1 &1 &3
\end{bmatrix}.
$$
\end{comment}

\begin{comment}
\item The new run is added within the i-th run of $\bfy$, for $1\le i \le  k$. In this case, the number of runs in $\bfx$ is $\rho(\bfx) = \rho(\bfy)+2=k+2$, and the run length profile of $\bfx$ is exactly the same as the one of $\bfy$ up to the $i$-th column, then the $i$-th run has length $s$ for some $s<r_i$, the $i+1$-th run has length $1$, and the $i+2$-th run has length $r_i-s$. For any $j>i+2$, the $j$-th run of $\bfx$ has the same length of the $(j-2)$-th run in $\bfy$. In our example for $i=k$ and $s=1$, $\bfx = 1110010101000$, and 
$$ \widehat{r}(\bfx)=
\begin{bmatrix}
1 & 0 & 1 & 0 & 1 & 0 & 1 &0\\
3 & 2 & 1 & 1& 1 & 1 &1 &3
\end{bmatrix}.
$$
\end{enumerate}

\textcolor{red}{To conclude, write how an insertion can alter the number of runs.}
\end{comment}


==> Intersection/r1.tex <==
This section is focused on Problem~\ref{prob3} and presents an explicit characterization of the intersection of $1$-deletion and $1$-insertion balls. Using these results, we solve Problems~\ref{prob1} and~\ref{prob4} for the case where the balls' radius is one. 

Since this section is focused on the specific case where $\bfy_1 \in \Sigma_q^{n-1}, \bfy_2 \in \Sigma_q^{n+1}$, and $d_L(\bfy_1, \bfy_2) = 2$, it holds that $\bfy_1$ can be obtained from $\bfy_2$ by exactly $2$ deletions. 
The following lemma states the possible options to receive $\bfy_1$ by $2$ deletions from $\bfy_2$. \vspace{-1ex}
%that $\bfy_1$ is obtained from $\bfy_2$ by either deleting two symbols from the same run of $\bfy_2$ or by deleting the two symbols from two distinct runs of $\bfy_2$ (but not both). 
%\begin{lemma} If $\bfy_1$ can be obtained from $\bfy_2$ by deleting two symbols from the same run of $\bfy_2$, then $\bfy_1$ can not be obtained from $\bfy_2$ by deleting the symbols from two distinct runs of $\bfy_2$. \end{lemma}
\begin{lemma} 
\label{lem: del location}
$\bfy_1$ can be obtained from $\bfy_2$ either by deleting two symbols from the same run, or by deleting them from two distinct runs, but not both.
\end{lemma}
%\vspace{-1ex}

The next definition will be used in characterizing the intersection size $\ID(\bfy_1,\bfy_2,n)$.%\vspace{-1.25ex}
\begin{definition} \label{def:R}
Let $\cR:\Sigma_q^{n-1}\times \Sigma_q^{n+1}\to \{0,1,2\}$ be defined as follows,%\vspace{-2.25ex}
\[
\cR(\bfy_1,\bfy_2) \triangleq \begin{cases}
0 & d_L(\bfy_1,\bfy_2)>2\\
1 & d_L(\bfy_1,\bfy_2)=2 \text{ and } \bfy_2\xrightarrow{1}\bfy_1\\
2 &  d_L(\bfy_1,\bfy_2)=2 \text{ and } \bfy_2\xrightarrow{2}\bfy_1,
\end{cases}
%\vspace{-1.25ex}
\]
where $ \bfy_2\xrightarrow{i}\bfy_1$ denotes the case where $\bfy_1$ can be obtained from $\bfy_2$ by deletion(s) from $i$ run(s).
\end{definition}
Lemma~\ref{lem: iff cond.} states that if $\cR(\bfy_1,\bfy_2)=0$, then $\ID(\bfy_1,\bfy_2,n)=\emptyset$. The size of $\ID(\bfy_1,\bfy_2,n)$ when $\cR(\bfy_1,\bfy_2)=1$ is given in the following lemma.
 
\begin{lemma}
\label{lem: R=1}
For $\bfy_1\in\Sigma_q^{n-1}, \bfy_2\in\Sigma_q^{n+1}$, if ${\cR(\bfy_1,\bfy_2)=1}$ then $\left|\ID(\bfy_1,\bfy_2,n)\right|=1$.
\end{lemma}
%\begin{IEEEproof}
%Since ${\cR(\bfy_1,\bfy_2)=1}$, there exists an index $1\le i \le \rho(\bfy_2)$ such that two symbols can be deleted from the $i$-th run of $\bfy_2$ to obtain $\bfy_1$. It can be verified that the only word in $\ID(\bfy_1,\bfy_2,n)$ is the word obtained from $\bfy_2$ by deleting one symbol from its $i$-th run.
%\end{IEEEproof}

To analyze the case where $\cR(\bfy_1,\bfy_2)=2$ we need to consider whether $\bfy_1$ can be obtained from $\bfy_2$ by deleting two consecutive runs or not. This will be done using the next definition. Note that this definition will be used in Theorem~\ref{the: ID size}, which is the main theorem of this section. 
\begin{definition} \label{def:A}
Let $\cA: \Sigma_q^{n-1}\times\Sigma_q^{n+1}\to \{0,1,\ldots, n-1\}$ be defined as follows. If $\bfy_1$ can be obtained from $\bfy_2$ by deleting two consecutive symbols and shortening a maximal alternating segment of $m$ symbols in $\bfy_2$ to a maximal alternating segment of $m-2$ symbols in $\bfy_1$ then $\cA(\bfy_1,\bfy_2) = m-2$, and $\cA(\bfy_1,\bfy_2) = 0$ otherwise.
\end{definition}
%\begin{figure}
%\includegraphics[width=\linewidth]{Picture1.png}
%\caption{An example of two sequences $\bfy_1$ and $\bfy_2$ and the set $\ID(\bfy_1,\bfy_2,n=10)$ (Theorem~\ref{the: ID size}). The bits that marked in blue represents the alternating segments that defines $\cA(\bfy_1,\bfy_2)=4$ (Definition~\ref{def:A}).}  \label{fig:example}
%\end{figure} 

%Figure~\ref{fig:example} presents an example for Definitions~\ref{def:R} and~\ref{def:A}. It can be seen that $|\bfy_1|=9, |\bfy_2|=11, n=10$, and that $d_L(\bfy_1, \bfy_2)=2$. Additionally, to obtain $\bfy_1$ from $\bfy_2$ deletions for two different runs are need and hence $\cR(\bfy_1,\bfy_2)=2$. The alternating segment that defines $\cA(\bfy_1,\bfy_2)$ is marked in blue. The length of this alternating segment is $6$ in $\bfy_2$, and  $4$ in $\bfy_1$ and therefore $\cA(\bfy_1,\bfy_2)=4$.  Lastly, Figure~\ref{fig:example} presents the set $\ID(\bfy_1, \bfy_2, n=10)$ which is of size 6 as proved in Theorem~\ref{the: ID size}.
 
For example, let $\bfy_1 = 0100\textcolor{blue}{0101}1$ and $\bfy_2 = 0100\textcolor{blue}{010101}1$. $\bfy_1$ can be obtained from $\bfy_2$ by deleting two consecutive symbols in the highlighted maximal alternating segment and hence $\cA(\bfy_1,\bfy_2)=6-2=4$. % Lastly, Figure~\ref{fig:example} presents the set $\ID(\bfy_1, \bfy_2, n=10)$ which is of size 6 as proved in Theorem~\ref{the: ID size}.

\begin{comment} 
\begin{lemma}
\label{lem: R=2 and equal rho}
Let $\bfy_1\in\Sigma_q^{n-1}$ and $\bfy_2\in\Sigma_q^{n+1}$ be two words. If  ${\cR(\bfy_1,\bfy_2)=2}$ and $\rho(\bfy_1)=\rho(\bfy_2)$ then $\ID(\bfy_1,\bfy_2,n)=2$.
\end{lemma}
\end{comment}

\begin{lemma}\label{lem: ID>2}
Let $\bfy_1\in\Sigma_q^{n-1}$ and $\bfy_2\in\Sigma_q^{n+1}$ be two words.\\ If $|\ID(\bfy_1,\bfy_2,n)|>2$ then $\cA(\bfy_1,\bfy_2)>0$.
\end{lemma} 

\begin{IEEEproof}
Let  $\bfy_1\in\Sigma_q^{n-1}$, $\bfy_2\in\Sigma_q^{n+1}$ be two words such that $|\ID(\bfy_1,\bfy_2,n)|>2$. Lemma~\ref{lem: R=1} implies that $\cR(\bfy_1,\bfy_2)=2$ and hence, there exist two indices $i < j$ such that $\bfy_1$ is obtained from $\bfy_2$ by deleting one symbol from the $i$-th run and one symbol from the $j$-th run of $\bfy_2$.
Assume that $i$ is the smallest such integer and that $j$ is the smallest integer with respect to $i$. Let $D_1(\bfy_2) = \{\bfx_1,\bfx_2,\dots,\bfx_{\rho(\bfy_2)}\}$, where $\bfx_k$ denotes the word obtained by deleting a symbol from the $k$-th run of $\bfy_2$. It is clear that $\bfx_i , \bfx_j$ are always supersequences of $\bfy_1$, since $\bfx_j$ is obtained by lengthening the run in $\bfy_1$ corresponding to the $i$-th run in $\bfy_2$, and vice versa. Since $|\ID(\bfy_1,\bfy_2,n)|>2$, there exists an index $\ell\ne i,j$ such that $\bfx_\ell$ is a supersequence of $\bfy_1$. Note that the minimality of $i$ implies that $\ell>i$. For $1\le k\le \rho(\bfy_2)$, let $\sigma_k$ be the symbol of the $k$-th run of $\bfy_2$ and $r_k$ is its length, i.e.,
$
\bfy_2 = \sigma_1^{r_1}\sigma_2^{r_2}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}}.
$
Assume to the contrary that  $\cA(\bfy_1,\bfy_2)=0$. By definition, the symbols from the $i$-th and $j$-th runs are not two consecutive symbols in a maximal alternating segment of length $m\ge 3$ in $\bfy_2$. Hence, we have the following distinct cases:\\
\textbf{Case 1:} If $i+1<j$, then we have that
\begin{align*}
\bfy_1 & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\textcolor{blue}{\sigma_i^{r_i-1}}\sigma_{i+1}^{r_{i+1}}\cdots \sigma_{j-1}^{r_{j-1}}\textcolor{blue}{\sigma_j^{r_j-1}}\sigma_{j+1}^{r_{j+1}}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}},\\
\bfx_\ell & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\sigma_i^{r_i}\cdots\sigma_\ell^{r_{\ell}-1}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}},
\end{align*}
where $\sigma^0$ is defined to be the empty word. 
Since $\bfx_\ell$ is a supersequence of $\bfy_1$, it can be verified that $\bfy_1$ must be obtained from $\bfx_\ell$ by deleting a symbol from the $i$-th run (with respect to the order of runs in $\bfy_2$). Hence, $\bfy_1$ can be obtained from $\bfx_i$ by deleting a symbol either from the $j$-th or the $\ell$-th run (with respect to their indices in $\bfy_2)$. This implies that the $j$-th and the $\ell$-th run of $\bfy_2$ are combined to a single run in $\bfx_i$. Thus, we have that either $j<i$ or $\ell < i$ which is a contradiction.\\
\textbf{Case 2:} If $i+1=j$, then $\ell>i,j$ and we have that
\begin{align*}
\bfy_1 & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\textcolor{blue}{\sigma_i^{r_i-1}\sigma_{i+1}^{r_{i+1}-1}}\sigma_{i+2}^{r_{i+2}}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}},\\
\bfx_\ell & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\sigma_i^{r_i}\sigma_{i+1}^{r_{i+1}}\cdots\sigma_\ell^{r_{\ell}-1}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}}.
\end{align*}
Let us prove that $\bfy_1$ is obtained from $\bfx_\ell$ by deleting a symbol from the $i$-th run (with respect to the order of runs in $\bfy_2$) which is a contradiction by the same arguments as in the previous case. 
If $r_{i}>1$ then clearly $\bfy_1$ is obtained from $\bfx_\ell$ by deleting a symbol from the $i$-th run. Otherwise, since $\cA(\bfy_1,\bfy_2)=0$, we have that $\sigma_{i-1}\ne\sigma_{i+1}$. If $r_{i+1}>1$ then again, $\bfy_1$ must be obtained from $\bfx_\ell$ by deleting a symbol from the $i$-th run. Otherwise, $r_{i+1}=1$ which implies that $\sigma_{i}\ne \sigma_{i+2}$ and we have that
\begin{align*}
\bfy_1 & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\sigma_{i+2}^{r_{i+2}}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}},\\
\bfx_\ell & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\sigma_i\sigma_{i+1}\cdots\sigma_\ell^{r_{\ell}-1}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}}.
\end{align*}
and since $\sigma_i\ne\sigma_{i+2}$, we conclude again that $\bfy_1$ is obtained from $\bfx_\ell$ by deleting a symbol from the $i$-th run. 
\end{IEEEproof}

\begin{comment}
\begin{IEEEproof}
Let $\bfy_1,\bfy_2$ be two words such that $|\ID(\bfy_1,\bfy_2,n)|>2$. Lemma~\ref{lem: R=1} implies that $\cR(\bfy_1,\bfy_2)=2$ and hence, there exist two indices $i < j$ such that $\bfy_1$ is obtained from $\bfy_2$ by deleting one symbol from the $i$-th run and one symbol from the $j$-th run of $\bfy_2$. Let $D_1(\bfy_2) = \{\bfx_1,\bfx_2,\dots,\bfx_{\rho(\bfy_2)}\}$, where $\bfx_k$ denotes the word obtained by deleting a symbol from the $k$-th run of $\bfy_2$. It is clear that $\bfx_i , \bfx_j$ are always supersequences of $\bfy_1$, since $\bfx_j$ is obtained by lengthening the run in $\bfy_1$ corresponding to the $i$-th run in $\bfy_2$, and vice versa. Since $|\ID(\bfy_1,\bfy_2,n)|>2$, there exists an index $\ell\ne i,j$ such that $\bfx_\ell$ is a supersequence of $\bfy_1$. For $1\le k\le \rho(\bfy_2)$, let $\sigma_k$ be the symbol of the $k$-th run of $\bfy_2$ and $r_k$ is its length, i.e.,
%$r_k$ denote the symbol, length of the $k$-th run of $\bfy_2$, respectively, i.e.,
\begin{align*}
\bfy_2 & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\sigma_i^{r_i}\sigma_{i+1}^{r_{i+1}}\cdots \sigma_{j-1}^{r_{j-1}}\sigma_j^{r_j}\sigma_{j+1}^{r_{j+1}}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}},\\
\bfy_1 & = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\textcolor{blue}{\sigma_i^{r_i-1}}\sigma_{i+1}^{r_{i+1}}\cdots \sigma_{j-1}^{r_{j-1}}\textcolor{blue}{\sigma_j^{r_j-1}}\sigma_{j+1}^{r_{j+1}}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}},
\end{align*}
where $\sigma^0$ is defined to be the empty word. 
First, we prove that $\ell < i$. Assume to the contrary that $i<\ell$, we have that, 
$$
\bfx_\ell = \sigma_1^{r_1}\cdots\sigma_{i-1}^{r_{i-1}}\sigma_i^{r_i}\cdots\sigma_\ell^{r_{\ell}-1}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}}.
$$
If $r_i>1$ or $\sigma_{i-1}\ne \sigma_{i+1}$ then $\bfy_1,\bfx_\ell$ are equal up to the $(i-1)$-th run and the $i$-th run of $\bfx_\ell$ is longer than the $i$-th run of $\bfy_1$ (if exists) by one. Hence, $\bfy_1$ must be obtained from $\bfx_\ell$ by deleting a symbol from the $i$-th run. 
If $r_i  \le 1$, we have that $r_i=1$, $\sigma_{i-1}= \sigma_{i+1}$ and $\bfy_1,\bfx_\ell$ are equal up to the $(i-2)$-th run and the $(i-1)$-th run of $\bfy_1$ is longer than the $(i-1)$-th run of $\bfx_\ell$ by $r_{i+1}$. 
It can be verified that since $\bfx_\ell$ is a supersequence of $\bfy_1$, $\bfy_1$ must be obtained from $\bfx_\ell$ by deleting a symbol from the $i$-th run, as before.  
Hence, $\bfy_1$ can be obtained from $\bfy_2$ by deleting one symbol from the $i$-th run and one more symbol, either from the $j$-th run or from the $\ell$-th run.  Since $\bfy_1$ can be obtained from $\bfx_i$ by deleting a symbol from the $j$-th or the $\ell$-th run (with respect to their indices in $\bfy_2)$, it holds that the $j$-th and the $\ell$-th run of $\bfy_2$ are combined to a single run in $\bfx_i$. This implies that either $j<i$ or $\ell < i$ which is a contradiction. 
%Assume w.l.o.g. that $j<\ell$, then the latter can be hold only if 
%$\sigma_i=\sigma_{\ell}$ 
%and $r_j=1$, that is, if $\sigma_i^{r_i}\sigma_j^{r_j}\sigma_{\ell}^{r_\ell} = \sigma_i^{r_i}\sigma_j\sigma_i^{r_{\ell}}$. Thus, by the definition of $\cA$,  we have that $\cA(\bfy_1,\bfy_2)>1$.\\

Next, since $\ell < i$ we have that 
\begin{align*}
& \bfx_\ell = \sigma_1^{r_1}\cdots\sigma_{\ell-1}^{r_{\ell-1}}\sigma_\ell^{r_\ell -1 }\cdots\sigma_i^{r_{i}}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}}, \\
& \bfy_1 = \sigma_1^{r_1}\cdots\sigma_{\ell-1}^{r_{\ell-1}}\textcolor{blue}{\sigma_\ell^{r_\ell}}\cdots {\sigma_i^{r_i-1}}\sigma_{i+1}^{r_{i+1}}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}}.
\end{align*}
If $r_\ell >1$ or $\sigma_{\ell-1} \ne \sigma_{\ell+1}$, then $\bfy_1,\bfx_\ell$ are equal up to the $(\ell-1)$-th run and the $\ell$-th run of $\bfy_1$ is longer than the $\ell$-th run of $\bfx_\ell$ (if exists) by one. Hence, $\bfy_1$ must be obtained from $\bfx_\ell$ by deleting a symbol from the $(\ell+1)$-th run, which must be of length one. Hence
$$
\sigma_\ell \sigma_{\ell+1}\cdots {\sigma_i^{r_i-1}}= \sigma_{\ell+2}\sigma_{\ell+3}\cdots \sigma_i^{r_{i}}\sigma_{i+1}
$$
and it can be verified that the last symbol of the $\ell$-th run and the first symbol of the $i$-th run are part of the same alternating segment of $\bfy_2$. If $i>\ell+1$ then this is an alternating segment of length three or more and by definition $\cA(\bfy_1,\bfy_2)>0$. Otherwise, $i=\ell+1$, and $\bfy_1$ is obtained from $\bfx_\ell$ by deleting one symbol from the $i$-th run and one symbol either from the $j$-th or from the $\ell$-th run of $\bfy_2$.  The latter can hold only if $i=\ell+1$, $j=\ell+2$ and $\sigma_\ell=\sigma_{j}$ which implies that $\cA(\bfy_1,\bfy_2)>0$. Otherwise, we have that $r_\ell=1$, $\sigma_{\ell-1}= \sigma_{\ell+1}$ and $\bfy_1,\bfx_\ell$ are equal up to the $(\ell-2)$-th run and the $(\ell-1)$-th run of $\bfx_\ell$ is longer than the $(\ell-1)$-th run of $\bfy_1$ by $r_{\ell+1}$. 
Since $\bfx_\ell$ is a supersequence of $\bfy_1$, $\bfy_1$ must be obtained from $\bfx_\ell$ by deleting a symbol from the $(\ell+1)$-th run, and by similar arguments, $\cA(\bfy_1,\bfy_2)>0$.  
\end{IEEEproof}
\begin{comment}
The following lemma is an immediate result of Lemma~\ref{lem: ID>2}. 
 
\begin{lemma}
\label{lem: R=2 and A=0}
Let $\bfy_1\in\Sigma_q^{n-1}$ and $\bfy_2\in\Sigma_q^{n+1}$ be two words. If  ${\cR(\bfy_1,\bfy_2)=2}$ and $\cA(\bfy_1,\bfy_2)=0$ then $\ID(\bfy_1,\bfy_2,n)=2$. 
\end{lemma}

\begin{comment}
Since $\cR(\bfy_1,\bfy_2)=2$, $\bfy_1$ is obtained from $\bfy_2$ by deleting two symbols from two different runs, one symbol from each. If both of these runs in $\bfy_2$ are of length $2$ or more, then, by Lemma~\ref{lem: R=2 and equal rho},  $\ID(\bfy_1,\bfy_2,n)=2$. Otherwise, at least one of the runs is of length one and $\rho(\bfy_1)<\rho(\bfy_2)$. Let $i \neq j$ be the indices of the runs the deletion occurred within (with respect to $\bfy_2$), such that the $i$-th run in $\bfy_2$ is of length 1. Let $D_1(\bfy_2) = \{\bfx_1,\bfx_2,\dots,\bfx_{\rho(\bfy_2)}\}$, where $\bfx_\ell$ denotes the word obtained by deleting a symbol from the $\ell$-th run. It is clear that $\bfx_i , \bfx_j$ are always supersequences of $\bfy_1$, since $\bfx_j$ is obtained by lengthening the run in $\bfy_1$ corresponding to the $i$-th run in $\bfy_2$, and vice versa.
It is left to show that for any $\ell\notin \{i,j\}$, $\bfx_\ell$ is not a supersequence of $\bfy_1$. Assume to the contrary that there exists an index $\ell\notin\{i,j\}$ such that $\bfx_\ell$ is a supersequence of $\bfy_1$. Let $\bfy_{i,\ell}$ denote the word which is obtained from  $\bfy_2$ by deleting one symbol from the $i$-th run and one symbol from the $\ell$-th run. Clearly, $\bfy_{i,\ell}\in D_1(\bfx_i)\cap D_1(\bfx_\ell)$ and since $\cA(\bfy_1,\bfy_2)=0$ it is possible $\bfy_1\ne \bfy_{i,\ell}$ we have that $|D_1(\bfx_i)\cap D_1(\bfx_\ell)|=2$. By similar arguments, we can also show  that $|D_1(\bfx_j)\cap D_1(\bfx_\ell)|=2$. By Lemma~\ref{lem: confusable}, both of the pairs, $\bfx_i,\bfx_\ell$ and $\bfx_j,\bfx_\ell$ are confusable. 
\end{comment}

\begin{comment}
For $1\le \ell\le \rho(\bfy_2)$, let $\sigma_\ell, r_\ell$ denote the symbol, length of the $\ell$-th run of $\bfy_2$, respectively. W.l.o.g. we have that 
\begin{align*}
\bfy_2 = \sigma_1^{r_1}\sigma_2^{r_2}\cdots\sigma_{i-1}^{r_{i-1}}\sigma_i\sigma_{i+1}^{r+1}\ldots \sigma_j^{r_j}\cdots \sigma_{\rho(\bfy_2)}^{r_{\rho(\bfy_2)}}.
\end{align*}
 If $\sigma_{i-1}=\sigma_{i+1}$, in the word $X_i$ the $(i-1)$-th and $(i+1)$-th runs (according to their enumeration in $\bfy_2$) are combined to a longer run
 Since $\cA(\bfy_1,\bfy_2)=0$ and the length of the $i$-th run is one, we have the following three distinct cases.\\
\textbf{Case $\bf 1$}: the length of the $j$-th run is greater than one.
\\
\textbf{Case $\bf 2$}: the length of the $j$-th run is one and $|i-j|>1$,
\textbf{Case $\bf 3$}: the length of the $j$-th run is one and $|i-j|=1$,
\end{comment}
 %\db{Since $\cA(\bfy_1,\bfy_2)=0$ and the length of the $i$-th run is one, it holds that if $j=i +1$ the length of the $j$-th run is necessarily greater than one.} Therefore, we have the following two distinct cases, the first one is the case where the $i$-th run in $\bfy_2$ stands between two other runs, and thus, in the word $X_i$ the $(i-1)$-th and $(i+1)$-th runs (according to their enumeration in $\bfy_2$) are combined to a longer run. The second case is where $i \in \{ 1, \rho(\bfy_2)\}$.  

 %in $\bfy_1$ \db{not necessarily, I think we need to consider the distinct cases}. 
 %Thus, for every $\ell \notin {i,j}$ we have that $\bfx_\ell \notin I_1(\bfy_1)$ and so $\ID(\bfy_1,\bfy_2,n)=2$. \db{TODO: complete proof}


\begin{comment}
We consider three distinct cases regarding the $i$-th and the $j$-th runs of $\bfy_2$.\\
\textbf{Case $1$} - If only one of the two runs is of length one. 
\\
\textbf{Case $2$} - both of the runs are of length one and $i<j-1$ (i.e, the runs are not consecutive).
\\
\textbf{Case $3$} -  both of the runs are of length one and $i=j-1$.
\end{comment}
The last case for $\bfy_1$ and $\bfy_2$ is handled in the next lemma.
\begin{lemma}
\label{lem: R=2 and A>0}
Let $\bfy_1\in\Sigma_q^{n-1}$ and $\bfy_2\in\Sigma_q^{n+1}$ be two words. If  ${\cR(\bfy_1,\bfy_2)=2}$ and $\cA(\bfy_1,\bfy_2)=m-2$ then ${\ID(\bfy_1,\bfy_2,n)=m}$.
\end{lemma}
\begin{IEEEproof}
By definition, $\bfy_1$ can be obtained from $\bfy_2$ by deleting two consecutive symbols from a maximal alternating segment of length $m$. 
Denote by $j,j+1,\ldots,j+m-1$ the indices of the runs which correspond to this maximal alternating segment. Let $D_1(\bfy_2) = \{\bfx_1,\bfx_2,\ldots , \bfx_{\rho(\bfy_2)}\}
$, where $\bfx_i$ is obtained from $\bfy_2$ by deleting one symbol from the $i$-th run of $\bfy_2$. It can be verified that for any $i\in\{j,\ldots, j+m-1\}$, $\bfy_1$ can be obtained from $\bfx_i$ by deleting a symbol from the $(i-1)$-th run or the $(i+1)$-th run of $\bfx_i$ (at least one of them is part of the maximal alternating segment). Hence $\bfx_i\in\ID(\bfy_1,\bfy_2,n)$. Otherwise, $i\notin \{j,\ldots, j+m-1\}$. Assume to the contrary that $\bfx_i$ is a supersequence of $\bfy_1$. By similar arguments  to those presented in the proof of Lemma~\ref{lem: ID>2}, it can be concluded that one of the symbols in the $i$-th run of $\bfy_2$ is part of the same alternating segment as the $j$-th run, which is a contradiction.
\end{IEEEproof}

\begin{theorem}\label{the: ID size}
For any two words $\bfy_1\in\Sigma_q^{n-1}$ and $\bfy_2\in\Sigma_q^{n+1}$, we have that \vspace{-1ex}
\[
\ID(\bfy_1,\bfy_2,n) = \cR(\bfy_1,\bfy_2) +  \cA(\bfy_1,\bfy_2).\vspace{-1ex}
\]
\end{theorem}
\begin{IEEEproof}
If $d_L(\bfy_1,\bfy_2)>2$ then by the definitions of $\cR,\cA$ we have that $\ID(\bfy_1,\bfy_2,n) = 0$.
Otherwise, by Lemma~\ref{lem: del location} it holds that either $ \bfy_2\xrightarrow{1}\bfy_1$ or  $\bfy_2\xrightarrow{2}\bfy_1$. 
If $ \bfy_2\xrightarrow{1}\bfy_1$ then by Lemma~\ref{lem: R=1}, $\ID(\bfy_1,\bfy_2,n) =1$ and by the definitions of $\cR,\cA$,
\[
 \cR(\bfy_1,\bfy_2) +  \cA(\bfy_1,\bfy_2) = 1 + 0 = 1
\]
Lastly, if $ \bfy_2\xrightarrow{2}\bfy_1$ then the result follows from Lemma~\ref{lem: ID>2} and Lemma~\ref{lem: R=2 and A>0}.
\end{IEEEproof}

\begin{corollary} \label{cor: max 1-intersection}
For any two integers $n,q>1$ we have that%\vspace{-1ex}
$$\max_{\substack{\bfy_1\in \Sigma_q^{n-1}, \bfy_2\in\Sigma_q^{n+1}}}|\ID(\bfy_1,\bfy_2,n)| = n+1,\vspace{-1ex}$$
and the maximum is obtained only when $\bfy_1$ and $\bfy_2$ are both alternating sequences consist from the same symbols $\sigma,\sigma'\in\Sigma_q$, and both start with $\sigma$.
%\begin{IEEEproof}
%By definition,  $0\le \cA(\bfy_1,\bfy_2)\le |\bfy_2|-2 = n-1$ and ${0\le \cR(\bfy_1,\bfy_2)\le 2}$. Hence, by Theorem~\ref{the: ID size}, 
 %$$|\ID(\bfy_1,\bfy_2,n)|  =  \cR(\bfy_1,\bfy_2) +  \cA(\bfy_1,\bfy_2) \le 2 + n-1 = n+1.$$
 %In addition, it can be verified that equality is obtained if and only if $\bfy_1$ is obtained from $\bfy_2$ by deleting two consecutive symbols from an alternating segment of length $n+1$ which completes the proof. 
%\end{IEEEproof}
\end{corollary} 

Note that the latter corollary is a generalization of Theorem~\ref{th:max} for any $q \ge 2$, where the balls' radius is one.  
Lastly, using Theorem~\ref{the: ID size}, it is possible to calculate the expected size of the set $\ID(\bfy_1,\bfy_2,n)$. The result is given in the next theorem.
%A generalization of Corollary~\ref{cor: max 1-intersection} for the binary case is given in the following theorem.

\begin{theorem} \label{th: exp 1-intersection}
For any two integers $n,q>1$ we have that%\vspace{-1ex}
$$\hspace{-3ex}\mathop{{}\mathbb{E}}_{\substack{\bfy_1\in \Sigma_q^{n-1}, \bfy_2\in\Sigma_q^{n+1}\\ \bfy_1 \text{ is a subsequence of } \bfy_2}}\hspace{-5.5ex}\left[|\ID(\bfy_1,\bfy_2,n)|\right] \hspace{-0.5ex}=\hspace{-0.5ex} 2-\dfrac{q}{1\hspace{-0.5ex}+\hspace{-0.5ex}(q\hspace{-0.5ex}-\hspace{-0.5ex}1)(n\hspace{-0.5ex}+\hspace{-0.5ex}1)\hspace{-0.5ex}+\hspace{-0.5ex}(q\hspace{-0.5ex}-\hspace{-0.5ex}1)^2\binom{n+1}{2}}.\vspace{-1ex}$$





\end{theorem} 
